Multicriteria Scalable Graph Drawing via Stochastic Gradient Descent, $(SGD)^2$

Readability criteria, such as distance or neighborhood preservation, are often used to optimize node-link representations of graphs to enable the comprehension of the underlying data. With few exceptions, graph drawing algorithms typically optimize one such criterion, usually at the expense of others. We propose a layout approach, Multicriteria Scalable Graph Drawing via Stochastic Gradient Descent, $(SGD)^2$, that can handle multiple readability criteria. $(SGD)^2$ can optimize any criterion that can be described by a differentiable function. Our approach is flexible and can be used to optimize several criteria that have already been considered earlier (e.g., obtaining ideal edge lengths, stress, neighborhood preservation) as well as other criteria which have not yet been explicitly optimized in such fashion (e.g., node resolution, angular resolution, aspect ratio). The approach is scalable and can handle large graphs. A variation of the underlying approach can also be used to optimize many desirable properties in planar graphs, while maintaining planarity. Finally, we provide quantitative and qualitative evidence of the effectiveness of $(SGD)^2$: we analyze the interactions between criteria, measure the quality of layouts generated from $(SGD)^2$ as well as the runtime behavior, and analyze the impact of sample sizes. The source code is available on github and we also provide an interactive demo for small graphs.

==> GD2/table-loss-functions.tex <==
\begin{table}[]
\resizebox{1.1\textwidth}{!}{
\centering
\begin{tabular}{p{2.0cm}|p{4cm}|p{4cm}|p{4cm}}
% \begin{tabular}{l|l|l|l|l}
% \begin{tabularx}{\textwidth}{X|l|l|l|l|l}
\toprule
Property 
& Gradient Descent 
& Subgradient Descent 
& Stochastic Gradient Descent\\
\midrule
Stress
 & $\sum\limits_{i<j}\;w_{ij}(|X_i - X_j|_2 - d_{ij})^2$ 
& $\sum\limits_{i<j}\;w_{ij}(|X_i - X_j|_2 - d_{ij})^2$ 
& $w_{ij}(|X_i - X_j|_2 - d_{ij})^2$ for a random pair of nodes $i, j \in V$\\ 
\hline



Ideal \hspace{.8cm}Edge Length
& $\sqrt{ \frac{1}{|E|} \sum\limits_{(i,j) \in E}\;  
(\frac{||X_i - X_j|| - l_{ij}}{l_{ij}}})^2$ (Eq.~\ref{eq:loss-ideal-edge-length})
& $\frac{1}{|E|} \sum\limits_{(i,j) \in E}\;  
|\frac{||X_i - X_j|| - l_{ij}}{l_{ij}}|$
& $|\frac{||X_i - X_j|| - l_{ij}}{l_{ij}}|$ for a random edge $(i,j) \in E$\\
\hline

Crossing \hspace{.5cm} Angle 
& $\sum\limits_i\;cos(\theta_i)^2$ 
& $\sum\limits_i\; |cos(\theta_i)|$
& $|cos(\theta_i)|$ for a random crossing $i$\\
\hline

Neighborhood Preservation
& Lov\'asz \textbf{softmax}~\cite{berman2018lovasz} between
  neighborhood prediction (Eq.\ref{eq:neighbor-pred})
  and adjacency matrix $Adj$
& Lov\'asz \textbf{hinge}~\cite{berman2018lovasz} between 
  neighborhood prediction (Eq.\ref{eq:neighbor-pred}) 
  and adjacency matrix $Adj$
& Lov\'asz \textbf{softmax} or \textbf{hinge}~\cite{berman2018lovasz} on a random node. 
  (i.e. Jaccard loss between a random \textit{row} of K in Eq. \ref{eq:neighbor-pred} 
  and the corresponding row in the adjacency matrix $Adj$)\\
\hline

Crossing Number
& Shabbeer et al.~\cite{bennett2010}
& Shabbeer et al.~\cite{bennett2010}
& Shabbeer et al.~\cite{bennett2010}\\
\hline

Angular \hspace{.5cm} Resolution
& $\sum\limits_{(i,j),(j,k) \in E}\; e^{-\varphi_{ijk}}$
& $\sum\limits_{v \in E}\; e^{-\varphi_{ijk}}$
& \makecell[l]{$e^{-\varphi_{ijk}}$ \\for random $(i,j),(j,k) \in E$} \\
\hline

Vertex\hspace{.8cm} Resolution
% &
& $\sum_{i,j \in V, i \neq j}$ ${ReLU( 1 - \frac{||X_i - X_j||}{d_{max} \cdot r}) ^2}$ (Eq. \ref{eq:loss-vertex-resolution})
& $\sum_{i,j \in V, i \neq j}$ ${ReLU( 1 - \frac{||X_i - X_j||}{d_{max} \cdot r})}$
& $ReLU( 1 - \frac{||X_i - X_j||}{d_{max} \cdot r})$ for random $i,j \in V, i \neq j$
\\
\hline

Gabriel Graph
&$\sum_{\substack{(i,j) \in E, k \in V \setminus \{i,j\}}} $ $ReLU(r_{ij} - |X_k - c_{ij}|) \; ^ 2$ (Eq. \ref{eq:gabriel})
&$\sum_{\substack{(i,j) \in E,k \in V \setminus \{i,j\}}} $ $ReLU(r_{ij} - |X_k - c_{ij}|)$
&$ReLU(r_{ij} - |X_k - c_{ij}|)$ for random $(i,j) \in E$ and $k \in V \setminus \{i,j\}$ 
\\
\hline

Aspect Ratio
& Eq. \ref{eq:aspect-ratio}
& Eq. \ref{eq:aspect-ratio}
& Eq. \ref{eq:aspect-ratio}
\\
% \hline
\bottomrule\\
% \end{tabularx}
\end{tabular}
} % resizebox end
\caption{Summary of the objective functions via different optimization methods.}
\label{table:loss-functions}
\end{table}

==> GD2/table-notations.tex <==
\begin{table}[h]
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|l}
    \toprule
    Notation & Description\\
    \midrule
    $G$ & Graph\\
    $V$ & The set of nodes in $G$, indexed by $i$, $j$ or $k$\\
    $E$ & The set of edges in $G$, indexed by a pair of nodes $i,j$ in $V$\\
    $n=|V|$ & Number of nodes in $G$\\
    $m$ & sample size for a certain criterion in SGD\\
    $|E|$ & Number of edges in $G$\\
    $Adj$ and $A_{i,j}$ & Adjacency matrix of $G$ and its $(i,j)$-th entry\\
    % $D$ & Graph-theoretic distance matrix\\
    $d_{ij}$ & Graph-theoretic distance between node $i$ and $j$\\
    $X_{n \times 2}$ & 2D-coordinates of nodes in the drawing\\
    $||X_i - X_j||$ & The Euclidean distance between nodes $i$ and $j$ \\
    $\theta_i$ & $i^{th}$ crossing angle\\
    $\varphi_{ijk}$ & Angle between incident edges $(i,j)$ and $(j,k)$\\
    % $c$ & A constant for angular resolution\\
    \bottomrule
    \end{tabular}
    \caption{Graph notation used in this paper.}
    \label{table:notations}
}
\end{table}

==> GD2/table-qualities-all.tex <==
%% ==== stress ====
\begin{table*}[thbp]
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.081          & \textbf{0.078} & \textbf{0.013} & \textbf{0.027} & 0.076          & \textbf{0.062} & 0.083          & \textbf{0.022} \\
 sfdp                          & 0.080 & 0.133          & 0.024          & 0.052          & 0.099          & 0.071          & \textbf{0.081} & 0.029          \\
 \GDGD (ST)                      & \textbf{0.079} & \textbf{0.078} & \textbf{0.013} & \textbf{0.027} & \textbf{0.071} & \textbf{0.062} & 0.082          & \textbf{0.022} \\
 \GDGD (NP)                      & 0.188          & 0.233          & 0.065          & 0.241          & 0.825          & 0.149          & 0.279          & 0.275          \\
 \GDGD (ST+IL)                   & 0.107          & 0.100          & 0.033          & 0.054          & 0.090          & 0.100          & 0.119          & 0.043          \\
 \GDGD (ST+NP)                   & 0.188          & 0.106          & \textbf{0.013} & 0.051          & 0.739          & 0.080          & 0.178          & 0.059          \\
 \GDGD (ST+CR)                   & 0.190          & \textbf{0.078} & \textbf{0.013} & 0.028          & 0.079          & 0.073          & 0.091          & 0.045          \\
 \GDGD (ST+CAM)                  & 0.099          & \textbf{0.078} & 0.015          & 0.029          & 0.075          & 0.063          & 0.094          & 0.029          \\
 \GDGD (ST+AR)                   & 0.080 & 0.081          & 0.055          & \textbf{0.027} & 0.075          & 0.067          & 0.084          & 0.023          \\
 \GDGD (ST+VR)                   & 0.083          & 0.080          & \textbf{0.013} & 0.032          & 0.073          & 0.063          & 0.088          & 0.023          \\
 \GDGD (ST+GB)                   & 0.080 & \textbf{0.078} & \textbf{0.013} & \textbf{0.027} & \textbf{0.071} & \textbf{0.062} & 0.083          & \textbf{0.022} \\
 \GDGD (ST+IL+ANR)               & 0.089          & 0.098          & 0.020          & 0.036          & 0.080          & 0.084          & 0.096          & 0.027          \\
 \GDGD (IL+NP+VR)                & 0.083          & 0.119          & 0.061          & 0.134          & 0.208          & 0.068          & 0.110          & 0.205          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Stress (ST)}}
\label{tab:quality-table-stress}
\end{table*}



%% ==== ideal_edge_length ====
\begin{table*}[thbp]
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.028          & 0.005          & \textbf{0.002} & 0.099          & 0.484          & 0.026          & 0.299          & 0.280          \\
 sfdp                          & 0.018          & 0.143          & 0.051          & 0.271          & 0.585          & 0.052          & 0.279          & 0.346          \\
 \GDGD (ST)                      & 0.062          & 0.103          & 0.053          & 0.114          & 0.526          & 0.111          & 0.320          & 0.293          \\
 \GDGD (NP)                      & 0.679          & 0.867          & 0.351          & 0.884          & 3.348          & 0.649          & 1.083          & 1.312          \\
 \GDGD (ST+IL)                   & \textbf{0.004} & \textbf{0.003} & \textbf{0.002} & \textbf{0.009} & \textbf{0.462} & \textbf{0.002} & \textbf{0.249} & \textbf{0.245} \\
 \GDGD (ST+NP)                   & 0.679          & 0.227          & 0.056          & 0.434          & 1.608          & 0.418          & 0.749          & 0.519          \\
 \GDGD (ST+CR)                   & 0.517          & 0.103          & 0.053          & 0.139          & 0.593          & 0.205          & 0.394          & 0.482          \\
 \GDGD (ST+CAM)                  & 0.109          & 0.103          & 0.058          & 0.132          & 0.595          & 0.141          & 0.497          & 0.368          \\
 \GDGD (ST+AR)                   & 0.061          & 0.112          & 0.203          & 0.114          & 0.533          & 0.148          & 0.334          & 0.302          \\
 \GDGD (ST+VR)                   & 0.083          & 0.257          & 0.067          & 0.159          & 0.569          & 0.155          & 0.399          & 0.309          \\
 \GDGD (ST+GB)                   & 0.061          & 0.098          & 0.053          & 0.092          & 0.521          & 0.111          & 0.338          & 0.291          \\
 \GDGD (ST+IL+ANR)               & 0.016          & 0.027          & 0.012          & 0.029          & 0.486          & 0.027          & 0.277          & 0.268          \\
 \GDGD (IL+NP+VR)                & 0.082          & 0.178          & 0.116          & 0.242          & 0.702          & 0.147          & 0.388          & 0.549          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Ideal Edge Length (IL)}}
\label{tab:quality-table-ideal_edge_length}
\end{table*}



%% ==== neighborhood_preservation ====
\begin{table*}[thbp]
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.723          & 0.718          & \textbf{0.000} & 0.474          & 0.846          & 0.558          & 0.699          & 0.545          \\
 sfdp                          & 0.571          & 0.592          & 0.063          & 0.533          & 0.750          & 0.651          & 0.584          & 0.653          \\
 \GDGD (ST)                      & 0.500          & 0.721          & \textbf{0.000} & 0.503          & 0.832          & 0.553          & 0.657          & 0.548          \\
 \GDGD (NP)                      & \textbf{0.400} & 0.225          & 0.276          & 0.487          & \textbf{0.659} & 0.480          & \textbf{0.428} & 0.516          \\
 \GDGD (ST+IL)                   & 0.667          & 0.701          & \textbf{0.000} & 0.518          & 0.867          & 0.674          & 0.766          & 0.665          \\
 \GDGD (ST+NP)                   & \textbf{0.400} & \textbf{0.194} & \textbf{0.000} & 0.467          & 0.664          & \textbf{0.347} & 0.472          & \textbf{0.441} \\
 \GDGD (ST+CR)                   & 0.481          & 0.714          & \textbf{0.000} & \textbf{0.420} & 0.765          & 0.532          & 0.582          & 0.567          \\
 \GDGD (ST+CAM)                  & 0.681          & 0.721          & 0.042          & 0.531          & 0.851          & 0.552          & 0.763          & 0.631          \\
 \GDGD (ST+AR)                   & 0.500          & 0.727          & 0.418          & 0.492          & 0.842          & 0.560          & 0.757          & 0.584          \\
 \GDGD (ST+VR)                   & 0.750          & 0.708          & \textbf{0.000} & 0.609          & 0.834          & 0.527          & 0.709          & 0.570          \\
 \GDGD (ST+GB)                   & 0.696          & 0.727          & \textbf{0.000} & 0.566          & 0.831          & 0.555          & 0.702          & 0.547          \\
 \GDGD (ST+IL+ANR)               & 0.500          & 0.749          & \textbf{0.000} & 0.539          & 0.823          & 0.622          & 0.705          & 0.520          \\
 \GDGD (IL+NP+VR)                & 0.636          & \textbf{0.194} & 0.165          & 0.472          & 0.713          & 0.349          & 0.497          & 0.717          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Neighborhood Preservation (NP)}}
\label{tab:quality-table-neighborhood_preservation}
\end{table*}



%% ==== crossings ====
\begin{table*}[thbp]
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron & tree-2-6   & grid-12-24 & spx-teaser  & 494-bus      & grid1       & dwt-307      & dwt-1005      \\
\hline
 neato                         & 8            & 1          & \textbf{0} & 80          & 274          & 134         & 1896         & 8001          \\
 sfdp                          & 9            & 2          & \textbf{0} & \textbf{72} & 141          & 109         & 1651         & \textbf{5447} \\
 \GDGD (ST)                      & 10           & \textbf{0} & \textbf{0} & 73          & 283          & 133         & 1749         & 8367          \\
 \GDGD (NP)                      & 10           & 5          & 109        & 155         & 216          & \textbf{80} & 1251         & 10736         \\
 \GDGD (ST+IL)                   & 10           & \textbf{0} & \textbf{0} & 73          & 325          & 151         & 3924         & 13094         \\
 \GDGD (ST+NP)                   & 6            & \textbf{0} & \textbf{0} & 111         & \textbf{131} & 94          & \textbf{265} & 6932          \\
 \GDGD (ST+CR)                   & \textbf{0}   & \textbf{0} & \textbf{0} & 73          & 187          & 133         & 347          & 8827          \\
 \GDGD (ST+CAM)                  & 7            & \textbf{0} & 9          & 84          & 430          & 158         & 4673         & 12972         \\
 \GDGD (ST+AR)                   & 10           & \textbf{0} & 2          & \textbf{72} & 303          & 142         & 2836         & 8628          \\
 \GDGD (ST+VR)                   & 7            & \textbf{0} & \textbf{0} & 79          & 282          & 134         & 2983         & 8874          \\
 \GDGD (ST+GB)                   & 6            & \textbf{0} & \textbf{0} & 75          & 264          & 134         & 2034         & 8305          \\
 \GDGD (ST+IL+ANR)               & 10           & 24         & \textbf{0} & \textbf{72} & 302          & 171         & 2793         & 8241          \\
 \GDGD (IL+NP+VR)                & 6            & 2          & 96         & 105         & 173          & 103         & 1333         & 18276         \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Crossings (CR)}}
\label{tab:quality-table-crossings}
\end{table*}



%% ==== crossing_angle_maximization ====
\begin{table*}[thbp]
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.254          & 0.419          & \textbf{0.000} & 0.786          & 0.956          & 0.927          & 0.970          & 0.999          \\
 sfdp                          & 0.622          & 0.235          & \textbf{0.000} & 0.806          & 0.972          & 0.970          & 0.963          & 1.000          \\
 \GDGD (ST)                      & 0.601          & \textbf{0.000} & \textbf{0.000} & 0.975          & 0.923          & 0.946          & 0.983          & 0.990          \\
 \GDGD (NP)                      & 0.969          & 0.808          & 0.945          & 0.999          & 0.913          & 0.939          & 0.988          & 0.992          \\
 \GDGD (ST+IL)                   & 0.602          & \textbf{0.000} & \textbf{0.000} & 0.575          & 0.970          & 0.837          & 0.989          & 0.998          \\
 \GDGD (ST+NP)                   & 0.969          & \textbf{0.000} & \textbf{0.000} & 1.000          & \textbf{0.838} & 0.864          & 0.958          & 0.992          \\
 \GDGD (ST+CR)                   & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & 0.940          & 0.885          & 0.889          & 0.955          & \textbf{0.984} \\
 \GDGD (ST+CAM)                  & \textbf{0.000} & \textbf{0.000} & 0.810          & 0.646          & 0.937          & \textbf{0.622} & 0.973          & 0.993          \\
 \GDGD (ST+AR)                   & 0.605          & \textbf{0.000} & 0.757          & 0.712          & 0.985          & 0.965          & 0.978          & 0.995          \\
 \GDGD (ST+VR)                   & 0.164          & \textbf{0.000} & \textbf{0.000} & 0.550          & 0.943          & 0.883          & 0.975          & 0.995          \\
 \GDGD (ST+GB)                   & 0.524          & \textbf{0.000} & \textbf{0.000} & 0.834          & 0.945          & 0.937          & 0.992          & 0.991          \\
 \GDGD (ST+IL+ANR)               & 0.603          & 0.725          & \textbf{0.000} & \textbf{0.421} & 0.935          & 0.961          & 0.973          & 0.997          \\
 \GDGD (IL+NP+VR)                & 0.323          & 0.143          & 0.954          & 0.963          & 0.913          & 0.631          & \textbf{0.926} & 0.991          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Crossing Angle Maximization (CAM)}}
\label{tab:quality-table-crossing_angle_maximization}
\end{table*}



%% ==== aspect_ratio ====
\begin{table*}[thbp]
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.062          & 0.145          & 0.483          & 0.010          & 0.143          & 0.314          & 0.065          & \textbf{0.012} \\
 sfdp                          & 0.068          & 0.084          & 0.536          & 0.010          & 0.192          & 0.452          & 0.095          & 0.018          \\
 \GDGD (ST)                      & 0.049          & 0.150          & 0.470          & \textbf{0.002} & 0.155          & 0.315          & 0.071          & 0.094          \\
 \GDGD (NP)                      & \textbf{0.047} & 0.124          & 0.481          & 0.176          & 0.162          & \textbf{0.049} & 0.109          & 0.282          \\
 \GDGD (ST+IL)                   & \textbf{0.048} & 0.169          & 0.507          & 0.018          & 0.160          & 0.470          & 0.157          & 0.045          \\
 \GDGD (ST+NP)                   & 0.049          & 0.126          & 0.479          & \textbf{0.002} & 0.192          & 0.209          & 0.077          & 0.101          \\
 \GDGD (ST+CR)                   & 0.134          & 0.149          & 0.473          & 0.028          & 0.136          & 0.368          & 0.030          & 0.079          \\
 \GDGD (ST+CAM)                  & 0.068          & 0.149          & 0.449          & 0.009          & 0.188          & 0.288          & \textbf{0.028} & 0.141          \\
 \GDGD (ST+AR)                   & \textbf{0.047} & \textbf{0.017} & \textbf{0.048} & 0.008          & \textbf{0.118} & 0.154          & 0.043          & 0.057          \\
 \GDGD (ST+VR)                   & 0.068          & 0.135          & 0.466          & 0.009          & 0.152          & 0.300          & 0.044          & 0.091          \\
 \GDGD (ST+GB)                   & 0.069          & 0.154          & 0.470          & 0.013          & 0.155          & 0.318          & 0.037          & 0.093          \\
 \GDGD (ST+IL+ANR)               & \textbf{0.048} & 0.197          & 0.508          & 0.045          & 0.178          & 0.269          & 0.058          & 0.084          \\
 \GDGD (IL+NP+VR)                & 0.101          & 0.231          & 0.455          & 0.242          & 0.359          & 0.282          & 0.074          & 0.106          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Aspect Ratio (AR)}}
\label{tab:quality-table-aspect_ratio}
\end{table*}



%% ==== angular_resolution ====
\begin{table*}[thbp]
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.753          & 0.749          & 0.525          & 0.999          & 0.998          & 1.000          & 1.000          & \textbf{1.000} \\
 sfdp                          & 0.459          & 0.908          & 0.547          & 0.996          & 0.999          & 0.996          & 1.000          & \textbf{1.000} \\
 \GDGD (ST)                      & \textbf{0.401} & 0.750          & 0.524          & 0.989          & \textbf{0.993} & 0.941          & 0.999          & \textbf{1.000} \\
 \GDGD (NP)                      & 0.928          & 0.976          & 0.994          & 0.996          & 1.000          & 0.984          & 1.000          & \textbf{1.000} \\
 \GDGD (ST+IL)                   & 0.517          & 0.844          & 0.497          & 0.939          & 0.999          & 0.932          & 0.999          & \textbf{1.000} \\
 \GDGD (ST+NP)                   & 0.952          & 0.466          & \textbf{0.487} & 1.000          & 0.999          & 0.998          & 0.999          & \textbf{1.000} \\
 \GDGD (ST+CR)                   & 0.746          & 0.769          & 0.526          & 0.996          & 0.998          & 0.969          & \textbf{0.998} & \textbf{0.999} \\
 \GDGD (ST+CAM)                  & 1.000          & 0.745          & 0.871          & 0.913          & 1.000          & 0.999          & 1.000          & \textbf{0.999} \\
 \GDGD (ST+AR)                   & 0.403          & 0.779          & 0.991          & 0.963          & 0.998          & 0.994          & 0.999          & \textbf{1.000} \\
 \GDGD (ST+VR)                   & 0.760          & 0.979          & 0.540          & 0.936          & 1.000          & 0.914          & 1.000          & \textbf{1.000} \\
 \GDGD (ST+GB)                   & 0.573          & 0.750          & 0.528          & \textbf{0.868} & 1.000          & 0.903          & 1.000          & \textbf{1.000} \\
 \GDGD (ST+IL+ANR)               & \textbf{0.401} & \textbf{0.327} & 0.528          & 0.990          & 1.000          & \textbf{0.740} & \textbf{0.999} & \textbf{0.999} \\
 \GDGD (IL+NP+VR)                & 0.677          & 0.418          & 0.974          & 0.995          & 0.999          & 0.823          & \textbf{0.999} & \textbf{1.000} \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Angular Resolution (ANR)}}
\label{tab:quality-table-angular_resolution}
\end{table*}



%% ==== vertex_resolution ====
\begin{table*}[thbp]
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.637          & 0.735          & 0.362          & 0.765          & 0.948          & 0.780          & 0.870          & \textbf{0.931} \\
 sfdp                          & 0.391          & 0.594          & 0.807          & 0.825          & 0.951          & 0.877          & 0.859          & 0.967          \\
 \GDGD (ST)                      & 0.269          & 0.727          & 0.368          & 0.663          & 0.991          & 0.798          & 0.869          & 0.976          \\
 \GDGD (NP)                      & 1.000          & 0.875          & 0.902          & 0.992          & 0.986          & 0.814          & 0.827          & 0.987          \\
 \GDGD (ST+IL)                   & 0.334          & 0.705          & \textbf{0.354} & 0.788          & 0.993          & 0.973          & 0.994          & 0.993          \\
 \GDGD (ST+NP)                   & 1.000          & 0.688          & 0.454          & 1.000          & 0.989          & 0.791          & 0.862          & 0.977          \\
 \GDGD (ST+CR)                   & 0.570          & 0.762          & 0.379          & 0.789          & 0.954          & 0.908          & 0.785          & 0.950          \\
 \GDGD (ST+CAM)                  & 0.996          & 0.715          & 0.839          & 0.789          & 0.974          & 0.856          & 0.967          & 0.959          \\
 \GDGD (ST+AR)                   & 0.278          & 0.682          & 0.633          & 0.698          & 0.938          & 0.802          & 0.963          & 0.991          \\
 \GDGD (ST+VR)                   & \textbf{0.165} & \textbf{0.266} & 0.388          & \textbf{0.407} & \textbf{0.754} & \textbf{0.590} & \textbf{0.617} & 0.945          \\
 \GDGD (ST+GB)                   & 0.529          & 0.737          & 0.365          & 0.630          & 0.895          & 0.858          & 0.913          & 0.986          \\
 \GDGD (ST+IL+ANR)               & 0.332          & 0.959          & 0.392          & 0.873          & 0.961          & 0.959          & 0.931          & 0.984          \\
 \GDGD (IL+NP+VR)                & 0.355          & 0.615          & 0.795          & 0.744          & 0.831          & \textbf{0.590} & 0.751          & 0.993          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Vertex Resolution (VR)}}
\label{tab:quality-table-vertex_resolution}
\end{table*}



%% ==== gabriel ====
\begin{table*}[thbp]
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.429          & 0.595          & \textbf{0.000} & 0.933          & \textbf{1.000} & 0.920          & \textbf{1.000} & \textbf{1.000} \\
 sfdp                          & 0.860          & 0.806          & 0.148          & 0.758          & \textbf{1.000} & 0.967          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST)                      & 0.677          & 0.130          & \textbf{0.000} & 0.795          & \textbf{1.000} & 0.963          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (NP)                      & 0.951          & 0.954          & 0.973          & 0.920          & \textbf{1.000} & 0.903          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+IL)                   & 0.679          & \textbf{0.000} & \textbf{0.000} & 0.834          & \textbf{1.000} & 0.860          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+NP)                   & 0.951          & 0.658          & \textbf{0.000} & \textbf{0.039} & \textbf{1.000} & 0.916          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+CR)                   & 0.704          & 0.205          & \textbf{0.000} & 0.967          & \textbf{1.000} & 0.988          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+CAM)                  & 0.695          & 0.199          & 0.799          & 0.836          & \textbf{1.000} & 0.905          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+AR)                   & 0.678          & 0.396          & 0.887          & 0.903          & \textbf{1.000} & 0.958          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+VR)                   & 0.437          & 0.957          & \textbf{0.000} & 0.862          & \textbf{1.000} & 0.987          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+GB)                   & \textbf{0.368} & 0.036          & \textbf{0.000} & 0.664          & \textbf{1.000} & \textbf{0.791} & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+IL+ANR)               & 0.681          & 0.745          & \textbf{0.000} & 0.630          & \textbf{1.000} & 0.967          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (IL+NP+VR)                & 0.421          & 0.800          & 0.982          & 0.926          & \textbf{1.000} & 0.972          & \textbf{1.000} & \textbf{1.000} \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Gabriel Property (GB)}}
\label{tab:quality-table-gabriel}
\end{table*}


==> GD2/table-qualities-old.tex <==
\begin{table}[H]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Crossings
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& \textbf{6.0} 
& \textbf{6.0} 
& 79.0 
& \cellcolor{yellow!50} \textbf{6.0} 
& \cellcolor{yellow!50} \textbf{6.0} 
& \cellcolor{green!50} 10.0 
 \\ \hline
cycle 
& \textbf{0.0} 
& \textbf{0.0} 
& 11.0 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
tree 
& \textbf{0.0} 
& \textbf{0.0} 
& 31.0 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
block 
& 23.0 
& \textbf{16.0} 
& 297.0 
& \cellcolor{yellow!50} 23.0 
& \cellcolor{yellow!50} \textbf{16.0} 
& \cellcolor{green!50} 25.0 
 \\ \hline
compl. 
& \textbf{3454} 
& 3571 
& 3572 
& \cellcolor{yellow!50} \textbf{3454} 
& \cellcolor{yellow!50} 3571 
& \cellcolor{yellow!50} 3572 
 \\ \hline
cube 
& \textbf{2.0} 
& \textbf{2.0} 
& 18.0 
& \cellcolor{yellow!50} \textbf{2.0} 
& \cellcolor{yellow!50} \textbf{2.0} 
& \cellcolor{green!50} \textbf{2.0} 
 \\ \hline
symme. 
& 1.0 
& \textbf{0.0} 
& 77.0 
& \cellcolor{yellow!50} 1.0 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
bipar. 
& \textbf{40.0} 
& 52.0 
& \textbf{40.0} 
& \cellcolor{yellow!50} \textbf{40.0} 
& \cellcolor{green!50} \textbf{40.0} 
& \cellcolor{yellow!50} \textbf{40.0} 
 \\ \hline
grid 
& \textbf{0.0} 
& \textbf{0.0} 
& 190.0 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
spx t. 
& 73.0 
& \textbf{71.0} 
& 7254.0 
& \cellcolor{yellow!50} 73.0 
& \cellcolor{yellow!50} \textbf{71.0} 
& \cellcolor{green!50} 76.0 
 \\ \hline
\end{tabular}
}
\end{minipage}
%\caption{The value of crossings of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
%\label{tab:avg_crossing_number}
%\end{table}
%\begin{table}[htpb]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Ideal edge length
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 0.14 
& 0.15 
& 0.53 
& \cellcolor{green!50} 0.1 
& \cellcolor{yellow!50} 0.15 
& \cellcolor{green!50} \textbf{0.08} 
 \\ \hline
cycle 
& \textbf{0.0} 
& \textbf{0.0} 
& 0.42 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
tree 
& \textbf{0.03} 
& 0.13 
& 0.31 
& \cellcolor{yellow!50} \textbf{0.03} 
& \cellcolor{green!50} 0.04 
& \cellcolor{green!50} 0.09 
 \\ \hline
block 
& 0.31 
& 0.43 
& 0.5 
& \cellcolor{green!50} \textbf{0.25} 
& \cellcolor{green!50} 0.33 
& \cellcolor{green!50} 0.31 
 \\ \hline
compl. 
& 0.42 
& \textbf{0.41} 
& 0.45 
& \cellcolor{green!50} \textbf{0.41} 
& \cellcolor{yellow!50} \textbf{0.41} 
& \cellcolor{green!50} \textbf{0.41} 
 \\ \hline
cube 
& 0.08 
& 0.12 
& 0.29 
& \cellcolor{green!50} 0.03 
& \cellcolor{green!50} \textbf{0.0} 
& \cellcolor{green!50} 0.12 
 \\ \hline
symme. 
& 0.08 
& 0.19 
& 0.46 
& \cellcolor{green!50} 0.07 
& \cellcolor{green!50} 0.05 
& \cellcolor{green!50} \textbf{0.04} 
 \\ \hline
bipar. 
& 0.31 
& 0.26 
& 0.44 
& \cellcolor{green!50} 0.16 
& \cellcolor{green!50} 0.13 
& \cellcolor{green!50} \textbf{0.1} 
 \\ \hline
grid 
& 0.01 
& 0.09 
& 0.41 
& \cellcolor{green!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
& \cellcolor{green!50} 0.01 
 \\ \hline
spx t. 
& 0.4 
& 0.32 
& 0.45 
& \cellcolor{green!50} 0.3 
& \cellcolor{green!50} \textbf{0.2} 
& \cellcolor{green!50} 0.32 
 \\ \hline
\end{tabular}
}
\end{minipage}
%\caption{The value of 
%ideal edge length
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_edge_uniformity}
%\end{table}
%\begin{table}[htpb]
\par\medskip
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Stress
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 21.4 
& 17.58 
& 111.05 
& \cellcolor{green!50} \textbf{17.45} 
& \cellcolor{yellow!50} 17.58 
& \cellcolor{green!50} 17.6 
 \\ \hline
cycle 
& \textbf{0.77} 
& \textbf{0.77} 
& 30.24 
& \cellcolor{yellow!50} \textbf{0.77} 
& \cellcolor{yellow!50} \textbf{0.77} 
& \cellcolor{green!50} \textbf{0.77} 
 \\ \hline
tree 
& \textbf{2.11} 
& 2.7 
& 98.49 
& \cellcolor{yellow!50} \textbf{2.11} 
& \cellcolor{green!50} 2.62 
& \cellcolor{green!50} 5.5 
 \\ \hline
block 
& 26.79 
& 28.22 
& 203.31 
& \cellcolor{green!50} 12.72 
& \cellcolor{green!50} 23.71 
& \cellcolor{green!50} \textbf{11.2} 
 \\ \hline
compl. 
& 33.54 
& 31.58 
& 37.87 
& \cellcolor{green!50} 31.53 
& \cellcolor{green!50} 31.49 
& \cellcolor{green!50} \textbf{31.47} 
 \\ \hline
cube 
& 2.75 
& 2.71 
& 11.69 
& \cellcolor{green!50} 2.66 
& \cellcolor{green!50} 2.69 
& \cellcolor{green!50} \textbf{2.65} 
 \\ \hline
symme. 
& 9.88 
& 5.38 
& 180.48 
& \cellcolor{yellow!50} 9.88 
& \cellcolor{green!50} \textbf{3.36} 
& \cellcolor{green!50} 3.97 
 \\ \hline
bipar. 
& 9.25 
& \textbf{8.5} 
& 12.48 
& \cellcolor{green!50} 8.52 
& \cellcolor{yellow!50} \textbf{8.5} 
& \cellcolor{green!50} 9.6 
 \\ \hline
grid 
& \textbf{6.77} 
& 7.38 
& 221.66 
& \cellcolor{yellow!50} \textbf{6.77} 
& \cellcolor{green!50} 6.78 
& \cellcolor{green!50} \textbf{6.77} 
 \\ \hline
spx t. 
& 674.8 
& 418.4 
& 9794 
& \cellcolor{green!50} \textbf{227.1} 
& \cellcolor{green!50} 235.3 
& \cellcolor{green!50} 227.2
 \\ \hline
\end{tabular}
}
\end{minipage}
%\caption{The value of 
%stress
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_stress}
%\end{table}
%\begin{table}[htpb]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Angular resolution
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 0.39 
& 0.39 
& 0.01 
& \cellcolor{green!50} \textbf{0.6} 
& \cellcolor{yellow!50} 0.39 
& \cellcolor{green!50} \textbf{0.6} 
 \\ \hline
cycle 
& \textbf{0.8} 
& \textbf{0.8} 
& 0.05 
& \cellcolor{yellow!50} \textbf{0.8} 
& \cellcolor{yellow!50} \textbf{0.8} 
& \cellcolor{green!50} \textbf{0.8} 
 \\ \hline
tree 
& 0.61 
& 0.56 
& 0.04 
& \cellcolor{green!50} 0.78 
& \cellcolor{green!50} 0.83 
& \cellcolor{green!50} \textbf{0.88} 
 \\ \hline
block 
& 0.05 
& 0.01 
& 0.0 
& \cellcolor{green!50} \textbf{0.36} 
& \cellcolor{green!50} 0.02 
& \cellcolor{green!50} 0.29 
 \\ \hline
compl. 
& 0.0 
& \textbf{0.01} 
& 0.0 
& \cellcolor{yellow!50} 0.0 
& \cellcolor{yellow!50} \textbf{0.01} 
& \cellcolor{yellow!50} 0.0 
 \\ \hline
cube 
& 0.28 
& 0.3 
& 0.01 
& \cellcolor{green!50} \textbf{0.46} 
& \cellcolor{green!50} 0.44 
& \cellcolor{green!50} 0.4 
 \\ \hline
symme. 
& 0.66 
& 0.6 
& 0.03 
& \cellcolor{green!50} 0.68 
& \cellcolor{green!50} 0.76 
& \cellcolor{green!50} \textbf{0.77} 
 \\ \hline
bipar. 
& 0.01 
& 0.03 
& 0.01 
& \cellcolor{green!50} 0.02 
& \cellcolor{green!50} 0.04 
& \cellcolor{green!50} \textbf{0.11} 
 \\ \hline
grid 
& 0.52 
& \textbf{0.54} 
& 0.0 
& \cellcolor{yellow!50} 0.52 
& \cellcolor{yellow!50} \textbf{0.54} 
& \cellcolor{green!50} 0.52 
 \\ \hline
spx t. 
& 0.02 
& 0.0 
& 0.0 
& \cellcolor{green!50} \textbf{0.03} 
& \cellcolor{yellow!50} 0.0 
& \cellcolor{yellow!50} 0.0 
 \\ \hline
\end{tabular}
}
\end{minipage}
\par\medskip
%\caption{The value of 
%angular resolution
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_angular_resolution}
%\end{table}
%\begin{table}[htpb]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Neighbor preservation
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 0.32 
& 0.3 
& 0.1 
& \cellcolor{green!50} \textbf{0.5} 
& \cellcolor{yellow!50} 0.3 
& \cellcolor{green!50} \textbf{0.5} 
 \\ \hline
cycle 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.08 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
tree 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.02 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
block 
& 0.57 
& 0.93 
& 0.12 
& \cellcolor{green!50} 0.83 
& \cellcolor{yellow!50} 0.93 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
compl. 
& \textbf{1.0} 
& \textbf{1.0} 
& \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
 \\ \hline
cube 
& \textbf{0.5} 
& \textbf{0.5} 
& 0.12 
& \cellcolor{yellow!50} \textbf{0.5} 
& \cellcolor{yellow!50} \textbf{0.5} 
& \cellcolor{green!50} \textbf{0.5} 
 \\ \hline
symme. 
& 0.75 
& 0.95 
& 0.05 
& \cellcolor{yellow!50} 0.75 
& \cellcolor{green!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
bipar. 
& \textbf{0.47} 
& \textbf{0.47} 
& 0.43 
& \cellcolor{yellow!50} \textbf{0.47} 
& \cellcolor{yellow!50} \textbf{0.47} 
& \cellcolor{yellow!50} 0.43 
 \\ \hline
grid 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.05 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
spx t. 
& 0.36 
& 0.44 
& 0.03 
& \cellcolor{green!50} 0.49 
& \cellcolor{green!50} 0.46 
& \cellcolor{green!50} \textbf{0.53} 
 \\ \hline
\end{tabular}
}
\end{minipage}
%\caption{The value of 
%neighbor preservation
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_neighbor}
%\end{table}
%\begin{table}[htpb]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Gabriel graph property
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 0.16 
& \textbf{0.64} 
& 0.07 
& \cellcolor{green!50} 0.32 
& \cellcolor{yellow!50} \textbf{0.64} 
& \cellcolor{green!50} 0.32 
 \\ \hline
cycle 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.29 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
tree 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.05 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
block 
& 0.16 
& 0.03 
& 0.04 
& \cellcolor{green!50} 0.57 
& \cellcolor{green!50} 0.14 
& \cellcolor{green!50} \textbf{0.59} 
 \\ \hline
compl. 
& 0.0 
& 0.01 
& 0.02 
& \cellcolor{green!50} 0.04 
& \cellcolor{yellow!50} 0.01 
& \cellcolor{green!50} \textbf{0.07} 
 \\ \hline
cube 
& 0.43 
& 0.51 
& 0.01 
& \cellcolor{green!50} 0.75 
& \cellcolor{green!50} \textbf{0.8} 
& \cellcolor{green!50} 0.71 
 \\ \hline
symme. 
& 0.54 
& \textbf{1.0} 
& 0.15 
& \cellcolor{green!50} 0.7 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
bipar. 
& 0.08 
& 0.11 
& 0.25 
& \cellcolor{green!50} 0.48 
& \cellcolor{green!50} 0.64 
& \cellcolor{green!50} \textbf{0.74} 
 \\ \hline
grid 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.03 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
spx t. 
& 0.04 
& 0.0 
& 0.02 
& \cellcolor{green!50} 0.06 
& \cellcolor{green!50} \textbf{0.08} 
& \cellcolor{green!50} \textbf{0.08} 
 \\ \hline
\end{tabular}
}
\end{minipage}
\par\medskip
%\caption{The value of 
%gabriel graph property
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_gabriel}
%\end{table}
%\begin{table}[htpb]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Node resolution
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 0.52 
& 0.54 
& 0.07 
& \cellcolor{green!50} 0.7 
& \cellcolor{green!50} \textbf{0.81} 
& \cellcolor{green!50} 0.68 
 \\ \hline
cycle 
& \textbf{0.98} 
& \textbf{0.98} 
& 0.32 
& \cellcolor{yellow!50} \textbf{0.98} 
& \cellcolor{yellow!50} \textbf{0.98} 
& \cellcolor{green!50} \textbf{0.98} 
 \\ \hline
tree 
& 0.68 
& 0.57 
& 0.23 
& \cellcolor{green!50} \textbf{0.69} 
& \cellcolor{green!50} 0.68 
& \cellcolor{green!50} 0.68 
 \\ \hline
block 
& 0.66 
& 0.38 
& 0.1 
& \cellcolor{green!50} \textbf{0.72} 
& \cellcolor{green!50} 0.59 
& \cellcolor{green!50} 0.51 
 \\ \hline
compl. 
& 0.8 
& \textbf{1.0} 
& 0.18 
& \cellcolor{green!50} 0.84 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} 0.91 
 \\ \hline
cube 
& 0.66 
& \textbf{0.82} 
& 0.11 
& \cellcolor{yellow!50} 0.66 
& \cellcolor{yellow!50} \textbf{0.82} 
& \cellcolor{green!50} 0.67 
 \\ \hline
symme. 
& 0.35 
& 0.43 
& 0.06 
& \cellcolor{green!50} 0.38 
& \cellcolor{green!50} 0.51 
& \cellcolor{green!50} \textbf{0.6} 
 \\ \hline
bipar. 
& 0.83 
& \textbf{0.87} 
& 0.21 
& \cellcolor{yellow!50} 0.83 
& \cellcolor{yellow!50} \textbf{0.87} 
& \cellcolor{green!50} 0.35 
 \\ \hline
grid 
& 0.87 
& 0.8 
& 0.08 
& \cellcolor{green!50} \textbf{0.88} 
& \cellcolor{green!50} \textbf{0.88} 
& \cellcolor{green!50} \textbf{0.88} 
 \\ \hline
spx t. 
& 0.47 
& \textbf{0.48} 
& 0.05 
& \cellcolor{yellow!50} 0.47 
& \cellcolor{yellow!50} \textbf{0.48} 
& \cellcolor{green!50} 0.32 
 \\ \hline
\end{tabular}
}
\end{minipage}
%\caption{The value of 
%vertex resolution
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_vertex_resolution}
%\end{table}
%\begin{table}[htpb]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Aspect ratio
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 0.92 
& 0.91 
& 0.88 
& \cellcolor{green!50} \textbf{0.96} 
& \cellcolor{green!50} \textbf{0.96} 
& \cellcolor{green!50} \textbf{0.96} 
 \\ \hline
cycle 
& \textbf{0.96} 
& 0.95 
& 0.67 
& \cellcolor{yellow!50} \textbf{0.96} 
& \cellcolor{yellow!50} 0.95 
& \cellcolor{green!50} \textbf{0.96} 
 \\ \hline
tree 
& 0.73 
& 0.67 
& \textbf{0.88} 
& \cellcolor{green!50} 0.86 
& \cellcolor{green!50} 0.76 
& \cellcolor{yellow!50} \textbf{0.88} 
 \\ \hline
block 
& 0.9 
& 0.74 
& 0.7 
& \cellcolor{green!50} \textbf{0.96} 
& \cellcolor{green!50} 0.9 
& \cellcolor{green!50} \textbf{0.96} 
 \\ \hline
compl. 
& 0.89 
& 0.97 
& 0.91 
& \cellcolor{green!50} \textbf{0.98} 
& \cellcolor{green!50} \textbf{0.98} 
& \cellcolor{green!50} \textbf{0.98} 
 \\ \hline
cube 
& 0.76 
& 0.79 
& 0.57 
& \cellcolor{green!50} 0.87 
& \cellcolor{yellow!50} 0.79 
& \cellcolor{green!50} \textbf{0.88} 
 \\ \hline
symme. 
& 0.58 
& 0.67 
& \textbf{0.89} 
& \cellcolor{green!50} 0.6 
& \cellcolor{yellow!50} 0.67 
& \cellcolor{yellow!50} \textbf{0.89} 
 \\ \hline
bipar. 
& 0.82 
& 0.9 
& \textbf{0.91} 
& \cellcolor{yellow!50} 0.82 
& \cellcolor{yellow!50} 0.9 
& \cellcolor{yellow!50} \textbf{0.91} 
 \\ \hline
grid 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.82 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
spx t. 
& 0.98 
& 0.86 
& 0.88 
& \cellcolor{green!50} \textbf{0.99} 
& \cellcolor{green!50} \textbf{0.99} 
& \cellcolor{green!50} \textbf{0.99} 
 \\ \hline
\end{tabular}
}
\end{minipage}
\par\medskip
%\caption{The value of 
%aspect ratio
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_aspect_ratio}
%\end{table}
%\begin{table}[htpb]
\centering
\begin{minipage}{.5\linewidth}
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Crossing angle
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& \textbf{0.06} 
& 0.12 
& 0.24 
& \cellcolor{yellow!50} \textbf{0.06} 
& \cellcolor{green!50} 0.09 
& \cellcolor{green!50} 0.15 
 \\ \hline
cycle 
& \textbf{0.0} 
& \textbf{0.0} 
& 0.19 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
tree 
& \textbf{0.0} 
& \textbf{0.0} 
& 0.23 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
block 
& 0.11 
& 0.1 
& 0.24 
& \cellcolor{green!50} \textbf{0.05} 
& \cellcolor{green!50} 0.06 
& \cellcolor{green!50} 0.09 
 \\ \hline
compl. 
& 0.25 
& \textbf{0.24} 
& \textbf{0.24} 
& \cellcolor{green!50} \textbf{0.24} 
& \cellcolor{yellow!50} \textbf{0.24} 
& \cellcolor{yellow!50} \textbf{0.24} 
 \\ \hline
cube 
& \textbf{0.03} 
& \textbf{0.03} 
& 0.21 
& \cellcolor{yellow!50} \textbf{0.03} 
& \cellcolor{yellow!50} \textbf{0.03} 
& \cellcolor{green!50} 0.04 
 \\ \hline
symme. 
& 0.03 
& \textbf{0.0} 
& 0.24 
& \cellcolor{yellow!50} 0.03 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
bipar. 
& \textbf{0.16} 
& 0.17 
& 0.23 
& \cellcolor{yellow!50} \textbf{0.16} 
& \cellcolor{yellow!50} 0.17 
& \cellcolor{green!50} 0.19 
 \\ \hline
grid 
& \textbf{0.0} 
& \textbf{0.0} 
& 0.23 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
spx t. 
& 0.16 
& 0.22 
& 0.25 
& \cellcolor{yellow!50} 0.16 
& \cellcolor{green!50} \textbf{0.15} 
& \cellcolor{green!50} 0.21 
 \\ \hline
\end{tabular}
}
\end{minipage}
\caption{The values of the nine criteria corresponding to the 10 graphs for the layouts computed by neato, sfdp, random, and 3 runs of \GDGD initialized with neato, sfdp, and random layouts. Bold values are the best. Green cells show an improvement, yellow cells show a tie,
 %, red cells show a decrease of the score 
 with respect to the initial values. {\color{red} Each table provides the scores of a single criterion. The name of the criterion optimized is mentioned in the title of the table. For example, the first table optimizes edge crossings.}
 }
\label{tab:avg_crossing_angle}
\end{table}

==> GD2/table-qualities-partial.tex <==
%% ==== stress ====
\begin{table*}[thbp]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.081          & \textbf{0.078} & \textbf{0.013} & \textbf{0.027} & 0.076          & \textbf{0.062} & 0.083          & \textbf{0.022} \\
 sfdp                          & 0.080 & 0.133          & 0.024          & 0.052          & 0.099          & 0.071          & \textbf{0.081} & 0.029          \\
 $(SGD)^2$ (ST)                & \textbf{0.079} & \textbf{0.078} & \textbf{0.013} & \textbf{0.027} & \textbf{0.071} & \textbf{0.062} & 0.082          & \textbf{0.022} \\
 $(SGD)^2$ (NP)                & 0.188          & 0.233          & 0.065          & 0.241          & 0.825          & 0.149          & 0.279          & 0.275          \\
 $(SGD)^2$ (ST+NP)             & 0.188          & 0.106          & \textbf{0.013} & 0.051          & 0.739          & 0.080          & 0.178          & 0.059          \\
 $(SGD)^2$ (ST+CR)             & 0.190          & \textbf{0.078} & \textbf{0.013} & 0.028          & 0.079          & 0.073          & 0.091          & 0.045          \\
 $(SGD)^2$ (ST+AR)             & 0.080 & 0.081          & 0.055          & \textbf{0.027} & 0.075          & 0.067          & 0.084          & 0.023          \\
 $(SGD)^2$ (ST+IL+ANR)         & 0.089          & 0.098          & 0.020          & 0.036          & 0.080          & 0.084          & 0.096          & 0.027          \\
 $(SGD)^2$ (IL+NP+VR)          & 0.083          & 0.119          & 0.061          & 0.134          & 0.208          & 0.068          & 0.110          & 0.205          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Stress}}
\label{tab:quality-table-stress}
\end{table*}



%% ==== ideal_edge_length ====
\begin{table*}[thbp]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.028          & \textbf{0.005} & \textbf{0.002} & 0.099          & \textbf{0.484} & \textbf{0.026} & 0.299          & 0.280          \\
 sfdp                          & 0.018          & 0.143          & 0.051          & 0.271          & 0.585          & 0.052          & 0.279          & 0.346          \\
 $(SGD)^2$ (ST)                & 0.062          & 0.103          & 0.053          & 0.114          & 0.526          & 0.111          & 0.320          & 0.293          \\
 $(SGD)^2$ (NP)                & 0.679          & 0.867          & 0.351          & 0.884          & 3.348          & 0.649          & 1.083          & 1.312          \\
 $(SGD)^2$ (ST+NP)             & 0.679          & 0.227          & 0.056          & 0.434          & 1.608          & 0.418          & 0.749          & 0.519          \\
 $(SGD)^2$ (ST+CR)             & 0.517          & 0.103          & 0.053          & 0.139          & 0.593          & 0.205          & 0.394          & 0.482          \\
 $(SGD)^2$ (ST+AR)             & 0.061          & 0.112          & 0.203          & 0.114          & 0.533          & 0.148          & 0.334          & 0.302          \\
 $(SGD)^2$ (ST+IL+ANR)         & \textbf{0.016} & 0.027          & 0.012          & \textbf{0.029} & 0.486          & 0.027          & \textbf{0.277} & \textbf{0.268} \\
 $(SGD)^2$ (IL+NP+VR)          & 0.082          & 0.178          & 0.116          & 0.242          & 0.702          & 0.147          & 0.388          & 0.549          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Ideal Edge Length}}
\label{tab:quality-table-ideal_edge_length}
\end{table*}



%% ==== neighborhood_preservation ====
\begin{table*}[thbp]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.723          & 0.718          & \textbf{0.000} & 0.474          & 0.846          & 0.558          & 0.699          & 0.545          \\
 sfdp                          & 0.571          & 0.592          & 0.063          & 0.533          & 0.750          & 0.651          & 0.584          & 0.653          \\
 $(SGD)^2$ (ST)                & 0.500          & 0.721          & \textbf{0.000} & 0.503          & 0.832          & 0.553          & 0.657          & 0.548          \\
 $(SGD)^2$ (NP)                & \textbf{0.400} & 0.225          & 0.276          & 0.487          & \textbf{0.659} & 0.480          & \textbf{0.428} & 0.516          \\
 $(SGD)^2$ (ST+NP)             & \textbf{0.400} & \textbf{0.194} & \textbf{0.000} & 0.467          & 0.664          & \textbf{0.347} & 0.472          & \textbf{0.441} \\
 $(SGD)^2$ (ST+CR)             & 0.481          & 0.714          & \textbf{0.000} & \textbf{0.420} & 0.765          & 0.532          & 0.582          & 0.567          \\
 $(SGD)^2$ (ST+AR)             & 0.500          & 0.727          & 0.418          & 0.492          & 0.842          & 0.560          & 0.757          & 0.584          \\
 $(SGD)^2$ (ST+IL+ANR)         & 0.500          & 0.749          & \textbf{0.000} & 0.539          & 0.823          & 0.622          & 0.705          & 0.520          \\
 $(SGD)^2$ (IL+NP+VR)          & 0.636          & \textbf{0.194} & 0.165          & 0.472          & 0.713          & 0.349          & 0.497          & 0.717          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Neighborhood Preservation}}
\label{tab:quality-table-neighborhood_preservation}
\end{table*}



%% ==== crossings ====
\begin{table*}[thbp]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron & tree-2-6   & grid-12-24 & spx-teaser  & 494-bus      & grid1       & dwt-307      & dwt-1005      \\
\hline
 neato                         & 8            & 1          & \textbf{0} & 80          & 274          & 134         & 1896         & 8001          \\
 sfdp                          & 9            & 2          & \textbf{0} & \textbf{72} & 141          & 109         & 1651         & \textbf{5447} \\
 $(SGD)^2$ (ST)                & 10           & \textbf{0} & \textbf{0} & 73          & 283          & 133         & 1749         & 8367          \\
 $(SGD)^2$ (NP)                & 10           & 5          & 109        & 155         & 216          & \textbf{80} & 1251         & 10736         \\
 $(SGD)^2$ (ST+NP)             & 6            & \textbf{0} & \textbf{0} & 111         & \textbf{131} & 94          & \textbf{265} & 6932          \\
 $(SGD)^2$ (ST+CR)             & \textbf{0}   & \textbf{0} & \textbf{0} & 73          & 187          & 133         & 347          & 8827          \\
 $(SGD)^2$ (ST+AR)             & 10           & \textbf{0} & 2          & \textbf{72} & 303          & 142         & 2836         & 8628          \\
 $(SGD)^2$ (ST+IL+ANR)         & 10           & 24         & \textbf{0} & \textbf{72} & 302          & 171         & 2793         & 8241          \\
 $(SGD)^2$ (IL+NP+VR)          & 6            & 2          & 96         & 105         & 173          & 103         & 1333         & 18276         \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Crossings}}
\label{tab:quality-table-crossings}
\end{table*}



% %% ==== crossing_angle_maximization ====
% \begin{table*}[thbp]
% \begin{tabular}{l|rrrrrrrr}
% \hline
%  methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
% \hline
%  neato                         & 0.254          & 0.419          & \textbf{0.000} & 0.786          & 0.956          & 0.927          & 0.970          & 0.999          \\
%  sfdp                          & 0.622          & 0.235          & \textbf{0.000} & 0.806          & 0.972          & 0.970          & 0.963          & 1.000          \\
%  $(SGD)^2$ (ST)                & 0.601          & \textbf{0.000} & \textbf{0.000} & 0.975          & 0.923          & 0.946          & 0.983          & 0.990          \\
%  $(SGD)^2$ (NP)                & 0.969          & 0.808          & 0.945          & 0.999          & 0.913          & 0.939          & 0.988          & 0.992          \\
%  $(SGD)^2$ (ST+NP)             & 0.969          & \textbf{0.000} & \textbf{0.000} & 1.000          & \textbf{0.838} & 0.864          & 0.958          & 0.992          \\
%  $(SGD)^2$ (ST+CR)             & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & 0.940          & 0.885          & 0.889          & 0.955          & \textbf{0.984} \\
%  $(SGD)^2$ (ST+AR)             & 0.605          & \textbf{0.000} & 0.757          & 0.712          & 0.985          & 0.965          & 0.978          & 0.995          \\
%  $(SGD)^2$ (ST+IL+ANR)         & 0.603          & 0.725          & \textbf{0.000} & \textbf{0.421} & 0.935          & 0.961          & 0.973          & 0.997          \\
%  $(SGD)^2$ (IL+NP+VR)          & 0.323          & 0.143          & 0.954          & 0.963          & 0.913          & \textbf{0.631} & \textbf{0.926} & 0.991          \\
% \hline
% \end{tabular}
% \caption{\blue{Quality Measures of Crossing Angle Maximization}}
% \label{tab:quality-table-crossing_angle_maximization}
% \end{table*}



% %% ==== aspect_ratio ====
% \begin{table*}[thbp]
% \begin{tabular}{l|rrrrrrrr}
% \hline
%  methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
% \hline
%  neato                         & 0.062          & 0.145          & 0.483          & 0.010          & 0.143          & 0.314          & 0.065          & \textbf{0.012} \\
%  sfdp                          & 0.068          & 0.084          & 0.536          & 0.010          & 0.192          & 0.452          & 0.095          & 0.018          \\
%  $(SGD)^2$ (ST)                & 0.049          & 0.150          & 0.470          & \textbf{0.002} & 0.155          & 0.315          & 0.071          & 0.094          \\
%  $(SGD)^2$ (NP)                & \textbf{0.047} & 0.124          & 0.481          & 0.176          & 0.162          & \textbf{0.049} & 0.109          & 0.282          \\
%  $(SGD)^2$ (ST+NP)             & 0.049          & 0.126          & 0.479          & \textbf{0.002} & 0.192          & 0.209          & 0.077          & 0.101          \\
%  $(SGD)^2$ (ST+CR)             & 0.134          & 0.149          & 0.473          & 0.028          & 0.136          & 0.368          & \textbf{0.030} & 0.079          \\
%  $(SGD)^2$ (ST+AR)             & \textbf{0.047} & \textbf{0.017} & \textbf{0.048} & 0.008          & \textbf{0.118} & 0.154          & 0.043          & 0.057          \\
%  $(SGD)^2$ (ST+IL+ANR)         & \textbf{0.048} & 0.197          & 0.508          & 0.045          & 0.178          & 0.269          & 0.058          & 0.084          \\
%  $(SGD)^2$ (IL+NP+VR)          & 0.101          & 0.231          & 0.455          & 0.242          & 0.359          & 0.282          & 0.074          & 0.106          \\
% \hline
% \end{tabular}
% \caption{\blue{Quality Measures of Aspect Ratio}}
% \label{tab:quality-table-aspect_ratio}
% \end{table*}



% %% ==== angular_resolution ====
% \begin{table*}[thbp]
% \begin{tabular}{l|rrrrrrrr}
% \hline
%  methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
% \hline
%  neato                         & 0.753          & 0.749          & 0.525          & 0.999          & 0.998          & 1.000          & 1.000          & \textbf{1.000} \\
%  sfdp                          & 0.459          & 0.908          & 0.547          & 0.996          & 0.999          & 0.996          & 1.000          & \textbf{1.000} \\
%  $(SGD)^2$ (ST)                & \textbf{0.401} & 0.750          & 0.524          & 0.989          & \textbf{0.993} & 0.941          & 0.999          & \textbf{1.000} \\
%  $(SGD)^2$ (NP)                & 0.928          & 0.976          & 0.994          & 0.996          & 1.000          & 0.984          & 1.000          & \textbf{1.000} \\
%  $(SGD)^2$ (ST+NP)             & 0.952          & 0.466          & \textbf{0.487} & 1.000          & 0.999          & 0.998          & 0.999          & \textbf{1.000} \\
%  $(SGD)^2$ (ST+CR)             & 0.746          & 0.769          & 0.526          & 0.996          & 0.998          & 0.969          & \textbf{0.998} & \textbf{0.999} \\
%  $(SGD)^2$ (ST+AR)             & 0.403          & 0.779          & 0.991          & \textbf{0.963} & 0.998          & 0.994          & 0.999          & \textbf{1.000} \\
%  $(SGD)^2$ (ST+IL+ANR)         & \textbf{0.401} & \textbf{0.327} & 0.528          & 0.990          & 1.000          & \textbf{0.740} & \textbf{0.999} & \textbf{0.999} \\
%  $(SGD)^2$ (IL+NP+VR)          & 0.677          & 0.418          & 0.974          & 0.995          & 0.999          & 0.823          & \textbf{0.999} & \textbf{1.000} \\
% \hline
% \end{tabular}
% \caption{\blue{Quality Measures of Angular Resolution}}
% \label{tab:quality-table-angular_resolution}
% \end{table*}



% %% ==== vertex_resolution ====
% \begin{table*}[thbp]
% \begin{tabular}{l|rrrrrrrr}
% \hline
%  methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
% \hline
%  neato                         & 0.637          & 0.735          & \textbf{0.362} & 0.765          & 0.948          & 0.780          & 0.870          & \textbf{0.931} \\
%  sfdp                          & 0.391          & \textbf{0.594} & 0.807          & 0.825          & 0.951          & 0.877          & 0.859          & 0.967          \\
%  $(SGD)^2$ (ST)                & \textbf{0.269} & 0.727          & 0.368          & \textbf{0.663} & 0.991          & 0.798          & 0.869          & 0.976          \\
%  $(SGD)^2$ (NP)                & 1.000          & 0.875          & 0.902          & 0.992          & 0.986          & 0.814          & 0.827          & 0.987          \\
%  $(SGD)^2$ (ST+NP)             & 1.000          & 0.688          & 0.454          & 1.000          & 0.989          & 0.791          & 0.862          & 0.977          \\
%  $(SGD)^2$ (ST+CR)             & 0.570          & 0.762          & 0.379          & 0.789          & 0.954          & 0.908          & 0.785          & 0.950          \\
%  $(SGD)^2$ (ST+AR)             & 0.278          & 0.682          & 0.633          & 0.698          & 0.938          & 0.802          & 0.963          & 0.991          \\
%  $(SGD)^2$ (ST+IL+ANR)         & 0.332          & 0.959          & 0.392          & 0.873          & 0.961          & 0.959          & 0.931          & 0.984          \\
%  $(SGD)^2$ (IL+NP+VR)          & 0.355          & 0.615          & 0.795          & 0.744          & \textbf{0.831} & \textbf{0.590} & \textbf{0.751} & 0.993          \\
% \hline
% \end{tabular}
% \caption{\blue{Quality Measures of Vertex Resolution}}
% \label{tab:quality-table-vertex_resolution}
% \end{table*}



% %% ==== gabriel ====
% \begin{table*}[thbp]
% \begin{tabular}{l|rrrrrrrr}
% \hline
%  methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
% \hline
%  neato                         & 0.429          & 0.595          & \textbf{0.000} & 0.933          & \textbf{1.000} & 0.920          & \textbf{1.000} & \textbf{1.000} \\
%  sfdp                          & 0.860          & 0.806          & 0.148          & 0.758          & \textbf{1.000} & 0.967          & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (ST)                & 0.677          & \textbf{0.130} & \textbf{0.000} & 0.795          & \textbf{1.000} & 0.963          & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (NP)                & 0.951          & 0.954          & 0.973          & 0.920          & \textbf{1.000} & \textbf{0.903} & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (ST+NP)             & 0.951          & 0.658          & \textbf{0.000} & \textbf{0.039} & \textbf{1.000} & 0.916          & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (ST+CR)             & 0.704          & 0.205          & \textbf{0.000} & 0.967          & \textbf{1.000} & 0.988          & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (ST+AR)             & 0.678          & 0.396          & 0.887          & 0.903          & \textbf{1.000} & 0.958          & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (ST+IL+ANR)         & 0.681          & 0.745          & \textbf{0.000} & 0.630          & \textbf{1.000} & 0.967          & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (IL+NP+VR)          & \textbf{0.421} & 0.800          & 0.982          & 0.926          & \textbf{1.000} & 0.972          & \textbf{1.000} & \textbf{1.000} \\
% \hline
% \end{tabular}
% \caption{\blue{Quality Measures of Gabriel}}
% \label{tab:quality-table-gabriel}
% \end{table*}

==> GD2/table-qualities.tex <==
%% ==== stress ====
\begin{table*}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.081          & \textbf{0.078} & \textbf{0.013} & \textbf{0.027} & 0.076          & \textbf{0.062} & 0.083          & \textbf{0.022} \\
 sfdp                          & 0.080 & 0.133          & 0.024          & 0.052          & 0.099          & 0.071          & \textbf{0.081} & 0.029          \\
 \GDGD (ST)                      & \textbf{0.079} & \textbf{0.078} & \textbf{0.013} & \textbf{0.027} & \textbf{0.071} & \textbf{0.062} & 0.082          & \textbf{0.022} \\
 \GDGD (NP)                      & 0.188          & 0.233          & 0.065          & 0.241          & 0.825          & 0.149          & 0.279          & 0.275          \\
 \GDGD (ST+IL)                   & 0.107          & 0.100          & 0.033          & 0.054          & 0.090          & 0.100          & 0.119          & 0.043          \\
 \GDGD (ST+NP)                   & 0.188          & 0.106          & \textbf{0.013} & 0.051          & 0.739          & 0.080          & 0.178          & 0.059          \\
 \GDGD (ST+CR)                   & 0.190          & \textbf{0.078} & \textbf{0.013} & 0.028          & 0.079          & 0.073          & 0.091          & 0.045          \\
 \GDGD (ST+CAM)                  & 0.099          & \textbf{0.078} & 0.015          & 0.029          & 0.075          & 0.063          & 0.094          & 0.029          \\
 \GDGD (ST+AR)                   & 0.080 & 0.081          & 0.055          & \textbf{0.027} & 0.075          & 0.067          & 0.084          & 0.023          \\
 \GDGD (ST+VR)                   & 0.083          & 0.080          & \textbf{0.013} & 0.032          & 0.073          & 0.063          & 0.088          & 0.023          \\
 \GDGD (ST+GB)                   & 0.080 & \textbf{0.078} & \textbf{0.013} & \textbf{0.027} & \textbf{0.071} & \textbf{0.062} & 0.083          & \textbf{0.022} \\
 \GDGD (ST+IL+ANR)               & 0.089          & 0.098          & 0.020          & 0.036          & 0.080          & 0.084          & 0.096          & 0.027          \\
 \GDGD (IL+NP+VR)                & 0.083          & 0.119          & 0.061          & 0.134          & 0.208          & 0.068          & 0.110          & 0.205          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Stress (ST)}}
\label{tab:quality-table-stress}
\end{table*}



%% ==== ideal_edge_length ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.028          & 0.005          & \textbf{0.002} & 0.099          & 0.484          & 0.026          & 0.299          & 0.280          \\
 sfdp                          & 0.018          & 0.143          & 0.051          & 0.271          & 0.585          & 0.052          & 0.279          & 0.346          \\
 \GDGD (ST)                      & 0.062          & 0.103          & 0.053          & 0.114          & 0.526          & 0.111          & 0.320          & 0.293          \\
 \GDGD (NP)                      & 0.679          & 0.867          & 0.351          & 0.884          & 3.348          & 0.649          & 1.083          & 1.312          \\
 \GDGD (ST+IL)                   & \textbf{0.004} & \textbf{0.003} & \textbf{0.002} & \textbf{0.009} & \textbf{0.462} & \textbf{0.002} & \textbf{0.249} & \textbf{0.245} \\
 \GDGD (ST+NP)                   & 0.679          & 0.227          & 0.056          & 0.434          & 1.608          & 0.418          & 0.749          & 0.519          \\
 \GDGD (ST+CR)                   & 0.517          & 0.103          & 0.053          & 0.139          & 0.593          & 0.205          & 0.394          & 0.482          \\
 \GDGD (ST+CAM)                  & 0.109          & 0.103          & 0.058          & 0.132          & 0.595          & 0.141          & 0.497          & 0.368          \\
 \GDGD (ST+AR)                   & 0.061          & 0.112          & 0.203          & 0.114          & 0.533          & 0.148          & 0.334          & 0.302          \\
 \GDGD (ST+VR)                   & 0.083          & 0.257          & 0.067          & 0.159          & 0.569          & 0.155          & 0.399          & 0.309          \\
 \GDGD (ST+GB)                   & 0.061          & 0.098          & 0.053          & 0.092          & 0.521          & 0.111          & 0.338          & 0.291          \\
 \GDGD (ST+IL+ANR)               & 0.016          & 0.027          & 0.012          & 0.029          & 0.486          & 0.027          & 0.277          & 0.268          \\
 \GDGD (IL+NP+VR)                & 0.082          & 0.178          & 0.116          & 0.242          & 0.702          & 0.147          & 0.388          & 0.549          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Ideal Edge Length (IL)}}
\label{tab:quality-table-ideal_edge_length}
\end{table}



%% ==== neighborhood_preservation ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.723          & 0.718          & \textbf{0.000} & 0.474          & 0.846          & 0.558          & 0.699          & 0.545          \\
 sfdp                          & 0.571          & 0.592          & 0.063          & 0.533          & 0.750          & 0.651          & 0.584          & 0.653          \\
 \GDGD (ST)                      & 0.500          & 0.721          & \textbf{0.000} & 0.503          & 0.832          & 0.553          & 0.657          & 0.548          \\
 \GDGD (NP)                      & \textbf{0.400} & 0.225          & 0.276          & 0.487          & \textbf{0.659} & 0.480          & \textbf{0.428} & 0.516          \\
 \GDGD (ST+IL)                   & 0.667          & 0.701          & \textbf{0.000} & 0.518          & 0.867          & 0.674          & 0.766          & 0.665          \\
 \GDGD (ST+NP)                   & \textbf{0.400} & \textbf{0.194} & \textbf{0.000} & 0.467          & 0.664          & \textbf{0.347} & 0.472          & \textbf{0.441} \\
 \GDGD (ST+CR)                   & 0.481          & 0.714          & \textbf{0.000} & \textbf{0.420} & 0.765          & 0.532          & 0.582          & 0.567          \\
 \GDGD (ST+CAM)                  & 0.681          & 0.721          & 0.042          & 0.531          & 0.851          & 0.552          & 0.763          & 0.631          \\
 \GDGD (ST+AR)                   & 0.500          & 0.727          & 0.418          & 0.492          & 0.842          & 0.560          & 0.757          & 0.584          \\
 \GDGD (ST+VR)                   & 0.750          & 0.708          & \textbf{0.000} & 0.609          & 0.834          & 0.527          & 0.709          & 0.570          \\
 \GDGD (ST+GB)                   & 0.696          & 0.727          & \textbf{0.000} & 0.566          & 0.831          & 0.555          & 0.702          & 0.547          \\
 \GDGD (ST+IL+ANR)               & 0.500          & 0.749          & \textbf{0.000} & 0.539          & 0.823          & 0.622          & 0.705          & 0.520          \\
 \GDGD (IL+NP+VR)                & 0.636          & \textbf{0.194} & 0.165          & 0.472          & 0.713          & 0.349          & 0.497          & 0.717          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Neighborhood Preservation (NP)}}
\label{tab:quality-table-neighborhood_preservation}
\end{table}



%% ==== crossings ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron & tree-2-6   & grid-12-24 & spx-teaser  & 494-bus      & grid1       & dwt-307      & dwt-1005      \\
\hline
 neato                         & 8            & 1          & \textbf{0} & 80          & 274          & 134         & 1896         & 8001          \\
 sfdp                          & 9            & 2          & \textbf{0} & \textbf{72} & 141          & 109         & 1651         & \textbf{5447} \\
 \GDGD (ST)                      & 10           & \textbf{0} & \textbf{0} & 73          & 283          & 133         & 1749         & 8367          \\
 \GDGD (NP)                      & 10           & 5          & 109        & 155         & 216          & \textbf{80} & 1251         & 10736         \\
 \GDGD (ST+IL)                   & 10           & \textbf{0} & \textbf{0} & 73          & 325          & 151         & 3924         & 13094         \\
 \GDGD (ST+NP)                   & 6            & \textbf{0} & \textbf{0} & 111         & \textbf{131} & 94          & \textbf{265} & 6932          \\
 \GDGD (ST+CR)                   & \textbf{0}   & \textbf{0} & \textbf{0} & 73          & 187          & 133         & 347          & 8827          \\
 \GDGD (ST+CAM)                  & 7            & \textbf{0} & 9          & 84          & 430          & 158         & 4673         & 12972         \\
 \GDGD (ST+AR)                   & 10           & \textbf{0} & 2          & \textbf{72} & 303          & 142         & 2836         & 8628          \\
 \GDGD (ST+VR)                   & 7            & \textbf{0} & \textbf{0} & 79          & 282          & 134         & 2983         & 8874          \\
 \GDGD (ST+GB)                   & 6            & \textbf{0} & \textbf{0} & 75          & 264          & 134         & 2034         & 8305          \\
 \GDGD (ST+IL+ANR)               & 10           & 24         & \textbf{0} & \textbf{72} & 302          & 171         & 2793         & 8241          \\
 \GDGD (IL+NP+VR)                & 6            & 2          & 96         & 105         & 173          & 103         & 1333         & 18276         \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Crossings (CR)}}
\label{tab:quality-table-crossings}
\end{table}



%% ==== crossing_angle_maximization ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.254          & 0.419          & \textbf{0.000} & 0.786          & 0.956          & 0.927          & 0.970          & 0.999          \\
 sfdp                          & 0.622          & 0.235          & \textbf{0.000} & 0.806          & 0.972          & 0.970          & 0.963          & 1.000          \\
 \GDGD (ST)                      & 0.601          & \textbf{0.000} & \textbf{0.000} & 0.975          & 0.923          & 0.946          & 0.983          & 0.990          \\
 \GDGD (NP)                      & 0.969          & 0.808          & 0.945          & 0.999          & 0.913          & 0.939          & 0.988          & 0.992          \\
 \GDGD (ST+IL)                   & 0.602          & \textbf{0.000} & \textbf{0.000} & 0.575          & 0.970          & 0.837          & 0.989          & 0.998          \\
 \GDGD (ST+NP)                   & 0.969          & \textbf{0.000} & \textbf{0.000} & 1.000          & \textbf{0.838} & 0.864          & 0.958          & 0.992          \\
 \GDGD (ST+CR)                   & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & 0.940          & 0.885          & 0.889          & 0.955          & \textbf{0.984} \\
 \GDGD (ST+CAM)                  & \textbf{0.000} & \textbf{0.000} & 0.810          & 0.646          & 0.937          & \textbf{0.622} & 0.973          & 0.993          \\
 \GDGD (ST+AR)                   & 0.605          & \textbf{0.000} & 0.757          & 0.712          & 0.985          & 0.965          & 0.978          & 0.995          \\
 \GDGD (ST+VR)                   & 0.164          & \textbf{0.000} & \textbf{0.000} & 0.550          & 0.943          & 0.883          & 0.975          & 0.995          \\
 \GDGD (ST+GB)                   & 0.524          & \textbf{0.000} & \textbf{0.000} & 0.834          & 0.945          & 0.937          & 0.992          & 0.991          \\
 \GDGD (ST+IL+ANR)               & 0.603          & 0.725          & \textbf{0.000} & \textbf{0.421} & 0.935          & 0.961          & 0.973          & 0.997          \\
 \GDGD (IL+NP+VR)                & 0.323          & 0.143          & 0.954          & 0.963          & 0.913          & 0.631          & \textbf{0.926} & 0.991          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Crossing Angle Maximization (CAM)}}
\label{tab:quality-table-crossing_angle_maximization}
\end{table}



%% ==== aspect_ratio ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.062          & 0.145          & 0.483          & 0.010          & 0.143          & 0.314          & 0.065          & \textbf{0.012} \\
 sfdp                          & 0.068          & 0.084          & 0.536          & 0.010          & 0.192          & 0.452          & 0.095          & 0.018          \\
 \GDGD (ST)                      & 0.049          & 0.150          & 0.470          & \textbf{0.002} & 0.155          & 0.315          & 0.071          & 0.094          \\
 \GDGD (NP)                      & \textbf{0.047} & 0.124          & 0.481          & 0.176          & 0.162          & \textbf{0.049} & 0.109          & 0.282          \\
 \GDGD (ST+IL)                   & \textbf{0.048} & 0.169          & 0.507          & 0.018          & 0.160          & 0.470          & 0.157          & 0.045          \\
 \GDGD (ST+NP)                   & 0.049          & 0.126          & 0.479          & \textbf{0.002} & 0.192          & 0.209          & 0.077          & 0.101          \\
 \GDGD (ST+CR)                   & 0.134          & 0.149          & 0.473          & 0.028          & 0.136          & 0.368          & 0.030          & 0.079          \\
 \GDGD (ST+CAM)                  & 0.068          & 0.149          & 0.449          & 0.009          & 0.188          & 0.288          & \textbf{0.028} & 0.141          \\
 \GDGD (ST+AR)                   & \textbf{0.047} & \textbf{0.017} & \textbf{0.048} & 0.008          & \textbf{0.118} & 0.154          & 0.043          & 0.057          \\
 \GDGD (ST+VR)                   & 0.068          & 0.135          & 0.466          & 0.009          & 0.152          & 0.300          & 0.044          & 0.091          \\
 \GDGD (ST+GB)                   & 0.069          & 0.154          & 0.470          & 0.013          & 0.155          & 0.318          & 0.037          & 0.093          \\
 \GDGD (ST+IL+ANR)               & \textbf{0.048} & 0.197          & 0.508          & 0.045          & 0.178          & 0.269          & 0.058          & 0.084          \\
 \GDGD (IL+NP+VR)                & 0.101          & 0.231          & 0.455          & 0.242          & 0.359          & 0.282          & 0.074          & 0.106          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Aspect Ratio (AR)}}
\label{tab:quality-table-aspect_ratio}
\end{table}



%% ==== angular_resolution ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.753          & 0.749          & 0.525          & 0.999          & 0.998          & 1.000          & 1.000          & \textbf{1.000} \\
 sfdp                          & 0.459          & 0.908          & 0.547          & 0.996          & 0.999          & 0.996          & 1.000          & \textbf{1.000} \\
 \GDGD (ST)                      & \textbf{0.401} & 0.750          & 0.524          & 0.989          & \textbf{0.993} & 0.941          & 0.999          & \textbf{1.000} \\
 \GDGD (NP)                      & 0.928          & 0.976          & 0.994          & 0.996          & 1.000          & 0.984          & 1.000          & \textbf{1.000} \\
 \GDGD (ST+IL)                   & 0.517          & 0.844          & 0.497          & 0.939          & 0.999          & 0.932          & 0.999          & \textbf{1.000} \\
 \GDGD (ST+NP)                   & 0.952          & 0.466          & \textbf{0.487} & 1.000          & 0.999          & 0.998          & 0.999          & \textbf{1.000} \\
 \GDGD (ST+CR)                   & 0.746          & 0.769          & 0.526          & 0.996          & 0.998          & 0.969          & \textbf{0.998} & \textbf{0.999} \\
 \GDGD (ST+CAM)                  & 1.000          & 0.745          & 0.871          & 0.913          & 1.000          & 0.999          & 1.000          & \textbf{0.999} \\
 \GDGD (ST+AR)                   & 0.403          & 0.779          & 0.991          & 0.963          & 0.998          & 0.994          & 0.999          & \textbf{1.000} \\
 \GDGD (ST+VR)                   & 0.760          & 0.979          & 0.540          & 0.936          & 1.000          & 0.914          & 1.000          & \textbf{1.000} \\
 \GDGD (ST+GB)                   & 0.573          & 0.750          & 0.528          & \textbf{0.868} & 1.000          & 0.903          & 1.000          & \textbf{1.000} \\
 \GDGD (ST+IL+ANR)               & \textbf{0.401} & \textbf{0.327} & 0.528          & 0.990          & 1.000          & \textbf{0.740} & \textbf{0.999} & \textbf{0.999} \\
 \GDGD (IL+NP+VR)                & 0.677          & 0.418          & 0.974          & 0.995          & 0.999          & 0.823          & \textbf{0.999} & \textbf{1.000} \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Angular Resolution (ANR)}}
\label{tab:quality-table-angular_resolution}
\end{table}



%% ==== vertex_resolution ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.637          & 0.735          & 0.362          & 0.765          & 0.948          & 0.780          & 0.870          & \textbf{0.931} \\
 sfdp                          & 0.391          & 0.594          & 0.807          & 0.825          & 0.951          & 0.877          & 0.859          & 0.967          \\
 \GDGD (ST)                      & 0.269          & 0.727          & 0.368          & 0.663          & 0.991          & 0.798          & 0.869          & 0.976          \\
 \GDGD (NP)                      & 1.000          & 0.875          & 0.902          & 0.992          & 0.986          & 0.814          & 0.827          & 0.987          \\
 \GDGD (ST+IL)                   & 0.334          & 0.705          & \textbf{0.354} & 0.788          & 0.993          & 0.973          & 0.994          & 0.993          \\
 \GDGD (ST+NP)                   & 1.000          & 0.688          & 0.454          & 1.000          & 0.989          & 0.791          & 0.862          & 0.977          \\
 \GDGD (ST+CR)                   & 0.570          & 0.762          & 0.379          & 0.789          & 0.954          & 0.908          & 0.785          & 0.950          \\
 \GDGD (ST+CAM)                  & 0.996          & 0.715          & 0.839          & 0.789          & 0.974          & 0.856          & 0.967          & 0.959          \\
 \GDGD (ST+AR)                   & 0.278          & 0.682          & 0.633          & 0.698          & 0.938          & 0.802          & 0.963          & 0.991          \\
 \GDGD (ST+VR)                   & \textbf{0.165} & \textbf{0.266} & 0.388          & \textbf{0.407} & \textbf{0.754} & \textbf{0.590} & \textbf{0.617} & 0.945          \\
 \GDGD (ST+GB)                   & 0.529          & 0.737          & 0.365          & 0.630          & 0.895          & 0.858          & 0.913          & 0.986          \\
 \GDGD (ST+IL+ANR)               & 0.332          & 0.959          & 0.392          & 0.873          & 0.961          & 0.959          & 0.931          & 0.984          \\
 \GDGD (IL+NP+VR)                & 0.355          & 0.615          & 0.795          & 0.744          & 0.831          & \textbf{0.590} & 0.751          & 0.993          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Vertex Resolution (VR)}}
\label{tab:quality-table-vertex_resolution}
\end{table}



%% ==== gabriel ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.429          & 0.595          & \textbf{0.000} & 0.933          & \textbf{1.000} & 0.920          & \textbf{1.000} & \textbf{1.000} \\
 sfdp                          & 0.860          & 0.806          & 0.148          & 0.758          & \textbf{1.000} & 0.967          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST)                      & 0.677          & 0.130          & \textbf{0.000} & 0.795          & \textbf{1.000} & 0.963          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (NP)                      & 0.951          & 0.954          & 0.973          & 0.920          & \textbf{1.000} & 0.903          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+IL)                   & 0.679          & \textbf{0.000} & \textbf{0.000} & 0.834          & \textbf{1.000} & 0.860          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+NP)                   & 0.951          & 0.658          & \textbf{0.000} & \textbf{0.039} & \textbf{1.000} & 0.916          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+CR)                   & 0.704          & 0.205          & \textbf{0.000} & 0.967          & \textbf{1.000} & 0.988          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+CAM)                  & 0.695          & 0.199          & 0.799          & 0.836          & \textbf{1.000} & 0.905          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+AR)                   & 0.678          & 0.396          & 0.887          & 0.903          & \textbf{1.000} & 0.958          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+VR)                   & 0.437          & 0.957          & \textbf{0.000} & 0.862          & \textbf{1.000} & 0.987          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+GB)                   & \textbf{0.368} & 0.036          & \textbf{0.000} & 0.664          & \textbf{1.000} & \textbf{0.791} & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+IL+ANR)               & 0.681          & 0.745          & \textbf{0.000} & 0.630          & \textbf{1.000} & 0.967          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (IL+NP+VR)                & 0.421          & 0.800          & 0.982          & 0.926          & \textbf{1.000} & 0.972          & \textbf{1.000} & \textbf{1.000} \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Gabriel Property (GB)}}
\label{tab:quality-table-gabriel}
\end{table}


==> table-loss-functions.tex <==
\begin{table}[]
\resizebox{1.1\textwidth}{!}{
\centering
\begin{tabular}{p{2.0cm}|p{4cm}|p{4cm}|p{4cm}}
% \begin{tabular}{l|l|l|l|l}
% \begin{tabularx}{\textwidth}{X|l|l|l|l|l}
\toprule
Property 
& Gradient Descent 
& Subgradient Descent 
& Stochastic Gradient Descent\\
\midrule
Stress
 & $\sum\limits_{i<j}\;w_{ij}(|X_i - X_j|_2 - d_{ij})^2$ 
& $\sum\limits_{i<j}\;w_{ij}(|X_i - X_j|_2 - d_{ij})^2$ 
& $w_{ij}(|X_i - X_j|_2 - d_{ij})^2$ for a random pair of nodes $i, j \in V$\\ 
\hline



Ideal \hspace{.8cm}Edge Length
& $\sqrt{ \frac{1}{|E|} \sum\limits_{(i,j) \in E}\;  
(\frac{||X_i - X_j|| - l_{ij}}{l_{ij}}})^2$ (Eq.~\ref{eq:loss-ideal-edge-length})
& $\frac{1}{|E|} \sum\limits_{(i,j) \in E}\;  
|\frac{||X_i - X_j|| - l_{ij}}{l_{ij}}|$
& $|\frac{||X_i - X_j|| - l_{ij}}{l_{ij}}|$ for a random edge $(i,j) \in E$\\
\hline

Crossing \hspace{.5cm} Angle 
& $\sum\limits_i\;cos(\theta_i)^2$ 
& $\sum\limits_i\; |cos(\theta_i)|$
& $|cos(\theta_i)|$ for a random crossing $i$\\
\hline

Neighborhood Preservation
& Lov\'asz \textbf{softmax}~\cite{berman2018lovasz} between
  neighborhood prediction (Eq.\ref{eq:neighbor-pred})
  and adjacency matrix $Adj$
& Lov\'asz \textbf{hinge}~\cite{berman2018lovasz} between 
  neighborhood prediction (Eq.\ref{eq:neighbor-pred}) 
  and adjacency matrix $Adj$
& Lov\'asz \textbf{softmax} or \textbf{hinge}~\cite{berman2018lovasz} on a random node. 
  (i.e. Jaccard loss between a random \textit{row} of K in Eq. \ref{eq:neighbor-pred} 
  and the corresponding row in the adjacency matrix $Adj$)\\
\hline

Crossing Number
& Shabbeer et al.~\cite{bennett2010}
& Shabbeer et al.~\cite{bennett2010}
& Shabbeer et al.~\cite{bennett2010}\\
\hline

Angular \hspace{.5cm} Resolution
& $\sum\limits_{(i,j),(j,k) \in E}\; e^{-\varphi_{ijk}}$
& $\sum\limits_{v \in E}\; e^{-\varphi_{ijk}}$
& \makecell[l]{$e^{-\varphi_{ijk}}$ \\for random $(i,j),(j,k) \in E$} \\
\hline

Vertex\hspace{.8cm} Resolution
% &
& $\sum_{i,j \in V, i \neq j}$ ${ReLU( 1 - \frac{||X_i - X_j||}{d_{max} \cdot r}) ^2}$ (Eq. \ref{eq:loss-vertex-resolution})
& $\sum_{i,j \in V, i \neq j}$ ${ReLU( 1 - \frac{||X_i - X_j||}{d_{max} \cdot r})}$
& $ReLU( 1 - \frac{||X_i - X_j||}{d_{max} \cdot r})$ for random $i,j \in V, i \neq j$
\\
\hline

Gabriel Graph
&$\sum_{\substack{(i,j) \in E, k \in V \setminus \{i,j\}}} $ $ReLU(r_{ij} - |X_k - c_{ij}|) \; ^ 2$ (Eq. \ref{eq:gabriel})
&$\sum_{\substack{(i,j) \in E,k \in V \setminus \{i,j\}}} $ $ReLU(r_{ij} - |X_k - c_{ij}|)$
&$ReLU(r_{ij} - |X_k - c_{ij}|)$ for random $(i,j) \in E$ and $k \in V \setminus \{i,j\}$ 
\\
\hline

Aspect Ratio
& Eq. \ref{eq:aspect-ratio}
& Eq. \ref{eq:aspect-ratio}
& Eq. \ref{eq:aspect-ratio}
\\
% \hline
\bottomrule\\
% \end{tabularx}
\end{tabular}
} % resizebox end
\caption{Summary of the objective functions via different optimization methods.}
\label{table:loss-functions}
\end{table}

==> table-qualities-old.tex <==
\begin{table}[H]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Crossings
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& \textbf{6.0} 
& \textbf{6.0} 
& 79.0 
& \cellcolor{yellow!50} \textbf{6.0} 
& \cellcolor{yellow!50} \textbf{6.0} 
& \cellcolor{green!50} 10.0 
 \\ \hline
cycle 
& \textbf{0.0} 
& \textbf{0.0} 
& 11.0 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
tree 
& \textbf{0.0} 
& \textbf{0.0} 
& 31.0 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
block 
& 23.0 
& \textbf{16.0} 
& 297.0 
& \cellcolor{yellow!50} 23.0 
& \cellcolor{yellow!50} \textbf{16.0} 
& \cellcolor{green!50} 25.0 
 \\ \hline
compl. 
& \textbf{3454} 
& 3571 
& 3572 
& \cellcolor{yellow!50} \textbf{3454} 
& \cellcolor{yellow!50} 3571 
& \cellcolor{yellow!50} 3572 
 \\ \hline
cube 
& \textbf{2.0} 
& \textbf{2.0} 
& 18.0 
& \cellcolor{yellow!50} \textbf{2.0} 
& \cellcolor{yellow!50} \textbf{2.0} 
& \cellcolor{green!50} \textbf{2.0} 
 \\ \hline
symme. 
& 1.0 
& \textbf{0.0} 
& 77.0 
& \cellcolor{yellow!50} 1.0 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
bipar. 
& \textbf{40.0} 
& 52.0 
& \textbf{40.0} 
& \cellcolor{yellow!50} \textbf{40.0} 
& \cellcolor{green!50} \textbf{40.0} 
& \cellcolor{yellow!50} \textbf{40.0} 
 \\ \hline
grid 
& \textbf{0.0} 
& \textbf{0.0} 
& 190.0 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
spx t. 
& 73.0 
& \textbf{71.0} 
& 7254.0 
& \cellcolor{yellow!50} 73.0 
& \cellcolor{yellow!50} \textbf{71.0} 
& \cellcolor{green!50} 76.0 
 \\ \hline
\end{tabular}
}
\end{minipage}
%\caption{The value of crossings of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
%\label{tab:avg_crossing_number}
%\end{table}
%\begin{table}[htpb]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Ideal edge length
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 0.14 
& 0.15 
& 0.53 
& \cellcolor{green!50} 0.1 
& \cellcolor{yellow!50} 0.15 
& \cellcolor{green!50} \textbf{0.08} 
 \\ \hline
cycle 
& \textbf{0.0} 
& \textbf{0.0} 
& 0.42 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
tree 
& \textbf{0.03} 
& 0.13 
& 0.31 
& \cellcolor{yellow!50} \textbf{0.03} 
& \cellcolor{green!50} 0.04 
& \cellcolor{green!50} 0.09 
 \\ \hline
block 
& 0.31 
& 0.43 
& 0.5 
& \cellcolor{green!50} \textbf{0.25} 
& \cellcolor{green!50} 0.33 
& \cellcolor{green!50} 0.31 
 \\ \hline
compl. 
& 0.42 
& \textbf{0.41} 
& 0.45 
& \cellcolor{green!50} \textbf{0.41} 
& \cellcolor{yellow!50} \textbf{0.41} 
& \cellcolor{green!50} \textbf{0.41} 
 \\ \hline
cube 
& 0.08 
& 0.12 
& 0.29 
& \cellcolor{green!50} 0.03 
& \cellcolor{green!50} \textbf{0.0} 
& \cellcolor{green!50} 0.12 
 \\ \hline
symme. 
& 0.08 
& 0.19 
& 0.46 
& \cellcolor{green!50} 0.07 
& \cellcolor{green!50} 0.05 
& \cellcolor{green!50} \textbf{0.04} 
 \\ \hline
bipar. 
& 0.31 
& 0.26 
& 0.44 
& \cellcolor{green!50} 0.16 
& \cellcolor{green!50} 0.13 
& \cellcolor{green!50} \textbf{0.1} 
 \\ \hline
grid 
& 0.01 
& 0.09 
& 0.41 
& \cellcolor{green!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
& \cellcolor{green!50} 0.01 
 \\ \hline
spx t. 
& 0.4 
& 0.32 
& 0.45 
& \cellcolor{green!50} 0.3 
& \cellcolor{green!50} \textbf{0.2} 
& \cellcolor{green!50} 0.32 
 \\ \hline
\end{tabular}
}
\end{minipage}
%\caption{The value of 
%ideal edge length
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_edge_uniformity}
%\end{table}
%\begin{table}[htpb]
\par\medskip
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Stress
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 21.4 
& 17.58 
& 111.05 
& \cellcolor{green!50} \textbf{17.45} 
& \cellcolor{yellow!50} 17.58 
& \cellcolor{green!50} 17.6 
 \\ \hline
cycle 
& \textbf{0.77} 
& \textbf{0.77} 
& 30.24 
& \cellcolor{yellow!50} \textbf{0.77} 
& \cellcolor{yellow!50} \textbf{0.77} 
& \cellcolor{green!50} \textbf{0.77} 
 \\ \hline
tree 
& \textbf{2.11} 
& 2.7 
& 98.49 
& \cellcolor{yellow!50} \textbf{2.11} 
& \cellcolor{green!50} 2.62 
& \cellcolor{green!50} 5.5 
 \\ \hline
block 
& 26.79 
& 28.22 
& 203.31 
& \cellcolor{green!50} 12.72 
& \cellcolor{green!50} 23.71 
& \cellcolor{green!50} \textbf{11.2} 
 \\ \hline
compl. 
& 33.54 
& 31.58 
& 37.87 
& \cellcolor{green!50} 31.53 
& \cellcolor{green!50} 31.49 
& \cellcolor{green!50} \textbf{31.47} 
 \\ \hline
cube 
& 2.75 
& 2.71 
& 11.69 
& \cellcolor{green!50} 2.66 
& \cellcolor{green!50} 2.69 
& \cellcolor{green!50} \textbf{2.65} 
 \\ \hline
symme. 
& 9.88 
& 5.38 
& 180.48 
& \cellcolor{yellow!50} 9.88 
& \cellcolor{green!50} \textbf{3.36} 
& \cellcolor{green!50} 3.97 
 \\ \hline
bipar. 
& 9.25 
& \textbf{8.5} 
& 12.48 
& \cellcolor{green!50} 8.52 
& \cellcolor{yellow!50} \textbf{8.5} 
& \cellcolor{green!50} 9.6 
 \\ \hline
grid 
& \textbf{6.77} 
& 7.38 
& 221.66 
& \cellcolor{yellow!50} \textbf{6.77} 
& \cellcolor{green!50} 6.78 
& \cellcolor{green!50} \textbf{6.77} 
 \\ \hline
spx t. 
& 674.8 
& 418.4 
& 9794 
& \cellcolor{green!50} \textbf{227.1} 
& \cellcolor{green!50} 235.3 
& \cellcolor{green!50} 227.2
 \\ \hline
\end{tabular}
}
\end{minipage}
%\caption{The value of 
%stress
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_stress}
%\end{table}
%\begin{table}[htpb]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Angular resolution
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 0.39 
& 0.39 
& 0.01 
& \cellcolor{green!50} \textbf{0.6} 
& \cellcolor{yellow!50} 0.39 
& \cellcolor{green!50} \textbf{0.6} 
 \\ \hline
cycle 
& \textbf{0.8} 
& \textbf{0.8} 
& 0.05 
& \cellcolor{yellow!50} \textbf{0.8} 
& \cellcolor{yellow!50} \textbf{0.8} 
& \cellcolor{green!50} \textbf{0.8} 
 \\ \hline
tree 
& 0.61 
& 0.56 
& 0.04 
& \cellcolor{green!50} 0.78 
& \cellcolor{green!50} 0.83 
& \cellcolor{green!50} \textbf{0.88} 
 \\ \hline
block 
& 0.05 
& 0.01 
& 0.0 
& \cellcolor{green!50} \textbf{0.36} 
& \cellcolor{green!50} 0.02 
& \cellcolor{green!50} 0.29 
 \\ \hline
compl. 
& 0.0 
& \textbf{0.01} 
& 0.0 
& \cellcolor{yellow!50} 0.0 
& \cellcolor{yellow!50} \textbf{0.01} 
& \cellcolor{yellow!50} 0.0 
 \\ \hline
cube 
& 0.28 
& 0.3 
& 0.01 
& \cellcolor{green!50} \textbf{0.46} 
& \cellcolor{green!50} 0.44 
& \cellcolor{green!50} 0.4 
 \\ \hline
symme. 
& 0.66 
& 0.6 
& 0.03 
& \cellcolor{green!50} 0.68 
& \cellcolor{green!50} 0.76 
& \cellcolor{green!50} \textbf{0.77} 
 \\ \hline
bipar. 
& 0.01 
& 0.03 
& 0.01 
& \cellcolor{green!50} 0.02 
& \cellcolor{green!50} 0.04 
& \cellcolor{green!50} \textbf{0.11} 
 \\ \hline
grid 
& 0.52 
& \textbf{0.54} 
& 0.0 
& \cellcolor{yellow!50} 0.52 
& \cellcolor{yellow!50} \textbf{0.54} 
& \cellcolor{green!50} 0.52 
 \\ \hline
spx t. 
& 0.02 
& 0.0 
& 0.0 
& \cellcolor{green!50} \textbf{0.03} 
& \cellcolor{yellow!50} 0.0 
& \cellcolor{yellow!50} 0.0 
 \\ \hline
\end{tabular}
}
\end{minipage}
\par\medskip
%\caption{The value of 
%angular resolution
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_angular_resolution}
%\end{table}
%\begin{table}[htpb]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Neighbor preservation
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 0.32 
& 0.3 
& 0.1 
& \cellcolor{green!50} \textbf{0.5} 
& \cellcolor{yellow!50} 0.3 
& \cellcolor{green!50} \textbf{0.5} 
 \\ \hline
cycle 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.08 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
tree 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.02 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
block 
& 0.57 
& 0.93 
& 0.12 
& \cellcolor{green!50} 0.83 
& \cellcolor{yellow!50} 0.93 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
compl. 
& \textbf{1.0} 
& \textbf{1.0} 
& \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
 \\ \hline
cube 
& \textbf{0.5} 
& \textbf{0.5} 
& 0.12 
& \cellcolor{yellow!50} \textbf{0.5} 
& \cellcolor{yellow!50} \textbf{0.5} 
& \cellcolor{green!50} \textbf{0.5} 
 \\ \hline
symme. 
& 0.75 
& 0.95 
& 0.05 
& \cellcolor{yellow!50} 0.75 
& \cellcolor{green!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
bipar. 
& \textbf{0.47} 
& \textbf{0.47} 
& 0.43 
& \cellcolor{yellow!50} \textbf{0.47} 
& \cellcolor{yellow!50} \textbf{0.47} 
& \cellcolor{yellow!50} 0.43 
 \\ \hline
grid 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.05 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
spx t. 
& 0.36 
& 0.44 
& 0.03 
& \cellcolor{green!50} 0.49 
& \cellcolor{green!50} 0.46 
& \cellcolor{green!50} \textbf{0.53} 
 \\ \hline
\end{tabular}
}
\end{minipage}
%\caption{The value of 
%neighbor preservation
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_neighbor}
%\end{table}
%\begin{table}[htpb]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Gabriel graph property
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 0.16 
& \textbf{0.64} 
& 0.07 
& \cellcolor{green!50} 0.32 
& \cellcolor{yellow!50} \textbf{0.64} 
& \cellcolor{green!50} 0.32 
 \\ \hline
cycle 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.29 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
tree 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.05 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
block 
& 0.16 
& 0.03 
& 0.04 
& \cellcolor{green!50} 0.57 
& \cellcolor{green!50} 0.14 
& \cellcolor{green!50} \textbf{0.59} 
 \\ \hline
compl. 
& 0.0 
& 0.01 
& 0.02 
& \cellcolor{green!50} 0.04 
& \cellcolor{yellow!50} 0.01 
& \cellcolor{green!50} \textbf{0.07} 
 \\ \hline
cube 
& 0.43 
& 0.51 
& 0.01 
& \cellcolor{green!50} 0.75 
& \cellcolor{green!50} \textbf{0.8} 
& \cellcolor{green!50} 0.71 
 \\ \hline
symme. 
& 0.54 
& \textbf{1.0} 
& 0.15 
& \cellcolor{green!50} 0.7 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
bipar. 
& 0.08 
& 0.11 
& 0.25 
& \cellcolor{green!50} 0.48 
& \cellcolor{green!50} 0.64 
& \cellcolor{green!50} \textbf{0.74} 
 \\ \hline
grid 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.03 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
spx t. 
& 0.04 
& 0.0 
& 0.02 
& \cellcolor{green!50} 0.06 
& \cellcolor{green!50} \textbf{0.08} 
& \cellcolor{green!50} \textbf{0.08} 
 \\ \hline
\end{tabular}
}
\end{minipage}
\par\medskip
%\caption{The value of 
%gabriel graph property
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_gabriel}
%\end{table}
%\begin{table}[htpb]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Node resolution
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 0.52 
& 0.54 
& 0.07 
& \cellcolor{green!50} 0.7 
& \cellcolor{green!50} \textbf{0.81} 
& \cellcolor{green!50} 0.68 
 \\ \hline
cycle 
& \textbf{0.98} 
& \textbf{0.98} 
& 0.32 
& \cellcolor{yellow!50} \textbf{0.98} 
& \cellcolor{yellow!50} \textbf{0.98} 
& \cellcolor{green!50} \textbf{0.98} 
 \\ \hline
tree 
& 0.68 
& 0.57 
& 0.23 
& \cellcolor{green!50} \textbf{0.69} 
& \cellcolor{green!50} 0.68 
& \cellcolor{green!50} 0.68 
 \\ \hline
block 
& 0.66 
& 0.38 
& 0.1 
& \cellcolor{green!50} \textbf{0.72} 
& \cellcolor{green!50} 0.59 
& \cellcolor{green!50} 0.51 
 \\ \hline
compl. 
& 0.8 
& \textbf{1.0} 
& 0.18 
& \cellcolor{green!50} 0.84 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} 0.91 
 \\ \hline
cube 
& 0.66 
& \textbf{0.82} 
& 0.11 
& \cellcolor{yellow!50} 0.66 
& \cellcolor{yellow!50} \textbf{0.82} 
& \cellcolor{green!50} 0.67 
 \\ \hline
symme. 
& 0.35 
& 0.43 
& 0.06 
& \cellcolor{green!50} 0.38 
& \cellcolor{green!50} 0.51 
& \cellcolor{green!50} \textbf{0.6} 
 \\ \hline
bipar. 
& 0.83 
& \textbf{0.87} 
& 0.21 
& \cellcolor{yellow!50} 0.83 
& \cellcolor{yellow!50} \textbf{0.87} 
& \cellcolor{green!50} 0.35 
 \\ \hline
grid 
& 0.87 
& 0.8 
& 0.08 
& \cellcolor{green!50} \textbf{0.88} 
& \cellcolor{green!50} \textbf{0.88} 
& \cellcolor{green!50} \textbf{0.88} 
 \\ \hline
spx t. 
& 0.47 
& \textbf{0.48} 
& 0.05 
& \cellcolor{yellow!50} 0.47 
& \cellcolor{yellow!50} \textbf{0.48} 
& \cellcolor{green!50} 0.32 
 \\ \hline
\end{tabular}
}
\end{minipage}
%\caption{The value of 
%vertex resolution
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_vertex_resolution}
%\end{table}
%\begin{table}[htpb]
\begin{minipage}{.5\linewidth}
\centering
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Aspect ratio
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& 0.92 
& 0.91 
& 0.88 
& \cellcolor{green!50} \textbf{0.96} 
& \cellcolor{green!50} \textbf{0.96} 
& \cellcolor{green!50} \textbf{0.96} 
 \\ \hline
cycle 
& \textbf{0.96} 
& 0.95 
& 0.67 
& \cellcolor{yellow!50} \textbf{0.96} 
& \cellcolor{yellow!50} 0.95 
& \cellcolor{green!50} \textbf{0.96} 
 \\ \hline
tree 
& 0.73 
& 0.67 
& \textbf{0.88} 
& \cellcolor{green!50} 0.86 
& \cellcolor{green!50} 0.76 
& \cellcolor{yellow!50} \textbf{0.88} 
 \\ \hline
block 
& 0.9 
& 0.74 
& 0.7 
& \cellcolor{green!50} \textbf{0.96} 
& \cellcolor{green!50} 0.9 
& \cellcolor{green!50} \textbf{0.96} 
 \\ \hline
compl. 
& 0.89 
& 0.97 
& 0.91 
& \cellcolor{green!50} \textbf{0.98} 
& \cellcolor{green!50} \textbf{0.98} 
& \cellcolor{green!50} \textbf{0.98} 
 \\ \hline
cube 
& 0.76 
& 0.79 
& 0.57 
& \cellcolor{green!50} 0.87 
& \cellcolor{yellow!50} 0.79 
& \cellcolor{green!50} \textbf{0.88} 
 \\ \hline
symme. 
& 0.58 
& 0.67 
& \textbf{0.89} 
& \cellcolor{green!50} 0.6 
& \cellcolor{yellow!50} 0.67 
& \cellcolor{yellow!50} \textbf{0.89} 
 \\ \hline
bipar. 
& 0.82 
& 0.9 
& \textbf{0.91} 
& \cellcolor{yellow!50} 0.82 
& \cellcolor{yellow!50} 0.9 
& \cellcolor{yellow!50} \textbf{0.91} 
 \\ \hline
grid 
& \textbf{1.0} 
& \textbf{1.0} 
& 0.82 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{yellow!50} \textbf{1.0} 
& \cellcolor{green!50} \textbf{1.0} 
 \\ \hline
spx t. 
& 0.98 
& 0.86 
& 0.88 
& \cellcolor{green!50} \textbf{0.99} 
& \cellcolor{green!50} \textbf{0.99} 
& \cellcolor{green!50} \textbf{0.99} 
 \\ \hline
\end{tabular}
}
\end{minipage}
\par\medskip
%\caption{The value of 
%aspect ratio
% of the 10 graphs for the layouts computed by neato, sfdp, random (rnd), \GDGD starting fron neato layouts ($(GD)^2_n$), \GDGD starting from sfdp layout ($(GD)^2_s$) and \GDGD starting from random layout ($(GD)^2_r$). Bold values are the best. Green cells show an increase, yellow cells show a tie, red cells show a decrease of the score with respect the initial value.}
\label{tab:avg_aspect_ratio}
%\end{table}
%\begin{table}[htpb]
\centering
\begin{minipage}{.5\linewidth}
{\tiny
\begin{tabular}{|l|l|l|l|l|l|l|} \hline
\multicolumn{7}{|c|}{
Crossing angle
}\\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{neato} & \multicolumn{1}{c|}{sdfp} & rnd & \multicolumn{1}{c|}{$(GD)^2_n$} & \multicolumn{1}{c|}{$(GD)^2_s$} & \multicolumn{1}{c|}{$(GD)^2_r$} \\ \hline
dodec. 
& \textbf{0.06} 
& 0.12 
& 0.24 
& \cellcolor{yellow!50} \textbf{0.06} 
& \cellcolor{green!50} 0.09 
& \cellcolor{green!50} 0.15 
 \\ \hline
cycle 
& \textbf{0.0} 
& \textbf{0.0} 
& 0.19 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
tree 
& \textbf{0.0} 
& \textbf{0.0} 
& 0.23 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
block 
& 0.11 
& 0.1 
& 0.24 
& \cellcolor{green!50} \textbf{0.05} 
& \cellcolor{green!50} 0.06 
& \cellcolor{green!50} 0.09 
 \\ \hline
compl. 
& 0.25 
& \textbf{0.24} 
& \textbf{0.24} 
& \cellcolor{green!50} \textbf{0.24} 
& \cellcolor{yellow!50} \textbf{0.24} 
& \cellcolor{yellow!50} \textbf{0.24} 
 \\ \hline
cube 
& \textbf{0.03} 
& \textbf{0.03} 
& 0.21 
& \cellcolor{yellow!50} \textbf{0.03} 
& \cellcolor{yellow!50} \textbf{0.03} 
& \cellcolor{green!50} 0.04 
 \\ \hline
symme. 
& 0.03 
& \textbf{0.0} 
& 0.24 
& \cellcolor{yellow!50} 0.03 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
bipar. 
& \textbf{0.16} 
& 0.17 
& 0.23 
& \cellcolor{yellow!50} \textbf{0.16} 
& \cellcolor{yellow!50} 0.17 
& \cellcolor{green!50} 0.19 
 \\ \hline
grid 
& \textbf{0.0} 
& \textbf{0.0} 
& 0.23 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{yellow!50} \textbf{0.0} 
& \cellcolor{green!50} \textbf{0.0} 
 \\ \hline
spx t. 
& 0.16 
& 0.22 
& 0.25 
& \cellcolor{yellow!50} 0.16 
& \cellcolor{green!50} \textbf{0.15} 
& \cellcolor{green!50} 0.21 
 \\ \hline
\end{tabular}
}
\end{minipage}
\caption{The values of the nine criteria corresponding to the 10 graphs for the layouts computed by neato, sfdp, random, and 3 runs of \GDGD initialized with neato, sfdp, and random layouts. Bold values are the best. Green cells show an improvement, yellow cells show a tie,
 %, red cells show a decrease of the score 
 with respect to the initial values. {\color{red} Each table provides the scores of a single criterion. The name of the criterion optimized is mentioned in the title of the table. For example, the first table optimizes edge crossings.}
 }
\label{tab:avg_crossing_angle}
\end{table}

==> table-qualities-partial.tex <==
%% ==== stress ====
\begin{table*}[thbp]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.081          & \textbf{0.078} & \textbf{0.013} & \textbf{0.027} & 0.076          & \textbf{0.062} & 0.083          & \textbf{0.022} \\
 sfdp                          & 0.080 & 0.133          & 0.024          & 0.052          & 0.099          & 0.071          & \textbf{0.081} & 0.029          \\
 $(SGD)^2$ (ST)                & \textbf{0.079} & \textbf{0.078} & \textbf{0.013} & \textbf{0.027} & \textbf{0.071} & \textbf{0.062} & 0.082          & \textbf{0.022} \\
 $(SGD)^2$ (NP)                & 0.188          & 0.233          & 0.065          & 0.241          & 0.825          & 0.149          & 0.279          & 0.275          \\
 $(SGD)^2$ (ST+NP)             & 0.188          & 0.106          & \textbf{0.013} & 0.051          & 0.739          & 0.080          & 0.178          & 0.059          \\
 $(SGD)^2$ (ST+CR)             & 0.190          & \textbf{0.078} & \textbf{0.013} & 0.028          & 0.079          & 0.073          & 0.091          & 0.045          \\
 $(SGD)^2$ (ST+AR)             & 0.080 & 0.081          & 0.055          & \textbf{0.027} & 0.075          & 0.067          & 0.084          & 0.023          \\
 $(SGD)^2$ (ST+IL+ANR)         & 0.089          & 0.098          & 0.020          & 0.036          & 0.080          & 0.084          & 0.096          & 0.027          \\
 $(SGD)^2$ (IL+NP+VR)          & 0.083          & 0.119          & 0.061          & 0.134          & 0.208          & 0.068          & 0.110          & 0.205          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Stress}}
\label{tab:quality-table-stress}
\end{table*}



%% ==== ideal_edge_length ====
\begin{table*}[thbp]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.028          & \textbf{0.005} & \textbf{0.002} & 0.099          & \textbf{0.484} & \textbf{0.026} & 0.299          & 0.280          \\
 sfdp                          & 0.018          & 0.143          & 0.051          & 0.271          & 0.585          & 0.052          & 0.279          & 0.346          \\
 $(SGD)^2$ (ST)                & 0.062          & 0.103          & 0.053          & 0.114          & 0.526          & 0.111          & 0.320          & 0.293          \\
 $(SGD)^2$ (NP)                & 0.679          & 0.867          & 0.351          & 0.884          & 3.348          & 0.649          & 1.083          & 1.312          \\
 $(SGD)^2$ (ST+NP)             & 0.679          & 0.227          & 0.056          & 0.434          & 1.608          & 0.418          & 0.749          & 0.519          \\
 $(SGD)^2$ (ST+CR)             & 0.517          & 0.103          & 0.053          & 0.139          & 0.593          & 0.205          & 0.394          & 0.482          \\
 $(SGD)^2$ (ST+AR)             & 0.061          & 0.112          & 0.203          & 0.114          & 0.533          & 0.148          & 0.334          & 0.302          \\
 $(SGD)^2$ (ST+IL+ANR)         & \textbf{0.016} & 0.027          & 0.012          & \textbf{0.029} & 0.486          & 0.027          & \textbf{0.277} & \textbf{0.268} \\
 $(SGD)^2$ (IL+NP+VR)          & 0.082          & 0.178          & 0.116          & 0.242          & 0.702          & 0.147          & 0.388          & 0.549          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Ideal Edge Length}}
\label{tab:quality-table-ideal_edge_length}
\end{table*}



%% ==== neighborhood_preservation ====
\begin{table*}[thbp]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.723          & 0.718          & \textbf{0.000} & 0.474          & 0.846          & 0.558          & 0.699          & 0.545          \\
 sfdp                          & 0.571          & 0.592          & 0.063          & 0.533          & 0.750          & 0.651          & 0.584          & 0.653          \\
 $(SGD)^2$ (ST)                & 0.500          & 0.721          & \textbf{0.000} & 0.503          & 0.832          & 0.553          & 0.657          & 0.548          \\
 $(SGD)^2$ (NP)                & \textbf{0.400} & 0.225          & 0.276          & 0.487          & \textbf{0.659} & 0.480          & \textbf{0.428} & 0.516          \\
 $(SGD)^2$ (ST+NP)             & \textbf{0.400} & \textbf{0.194} & \textbf{0.000} & 0.467          & 0.664          & \textbf{0.347} & 0.472          & \textbf{0.441} \\
 $(SGD)^2$ (ST+CR)             & 0.481          & 0.714          & \textbf{0.000} & \textbf{0.420} & 0.765          & 0.532          & 0.582          & 0.567          \\
 $(SGD)^2$ (ST+AR)             & 0.500          & 0.727          & 0.418          & 0.492          & 0.842          & 0.560          & 0.757          & 0.584          \\
 $(SGD)^2$ (ST+IL+ANR)         & 0.500          & 0.749          & \textbf{0.000} & 0.539          & 0.823          & 0.622          & 0.705          & 0.520          \\
 $(SGD)^2$ (IL+NP+VR)          & 0.636          & \textbf{0.194} & 0.165          & 0.472          & 0.713          & 0.349          & 0.497          & 0.717          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Neighborhood Preservation}}
\label{tab:quality-table-neighborhood_preservation}
\end{table*}



%% ==== crossings ====
\begin{table*}[thbp]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron & tree-2-6   & grid-12-24 & spx-teaser  & 494-bus      & grid1       & dwt-307      & dwt-1005      \\
\hline
 neato                         & 8            & 1          & \textbf{0} & 80          & 274          & 134         & 1896         & 8001          \\
 sfdp                          & 9            & 2          & \textbf{0} & \textbf{72} & 141          & 109         & 1651         & \textbf{5447} \\
 $(SGD)^2$ (ST)                & 10           & \textbf{0} & \textbf{0} & 73          & 283          & 133         & 1749         & 8367          \\
 $(SGD)^2$ (NP)                & 10           & 5          & 109        & 155         & 216          & \textbf{80} & 1251         & 10736         \\
 $(SGD)^2$ (ST+NP)             & 6            & \textbf{0} & \textbf{0} & 111         & \textbf{131} & 94          & \textbf{265} & 6932          \\
 $(SGD)^2$ (ST+CR)             & \textbf{0}   & \textbf{0} & \textbf{0} & 73          & 187          & 133         & 347          & 8827          \\
 $(SGD)^2$ (ST+AR)             & 10           & \textbf{0} & 2          & \textbf{72} & 303          & 142         & 2836         & 8628          \\
 $(SGD)^2$ (ST+IL+ANR)         & 10           & 24         & \textbf{0} & \textbf{72} & 302          & 171         & 2793         & 8241          \\
 $(SGD)^2$ (IL+NP+VR)          & 6            & 2          & 96         & 105         & 173          & 103         & 1333         & 18276         \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Crossings}}
\label{tab:quality-table-crossings}
\end{table*}



% %% ==== crossing_angle_maximization ====
% \begin{table*}[thbp]
% \begin{tabular}{l|rrrrrrrr}
% \hline
%  methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
% \hline
%  neato                         & 0.254          & 0.419          & \textbf{0.000} & 0.786          & 0.956          & 0.927          & 0.970          & 0.999          \\
%  sfdp                          & 0.622          & 0.235          & \textbf{0.000} & 0.806          & 0.972          & 0.970          & 0.963          & 1.000          \\
%  $(SGD)^2$ (ST)                & 0.601          & \textbf{0.000} & \textbf{0.000} & 0.975          & 0.923          & 0.946          & 0.983          & 0.990          \\
%  $(SGD)^2$ (NP)                & 0.969          & 0.808          & 0.945          & 0.999          & 0.913          & 0.939          & 0.988          & 0.992          \\
%  $(SGD)^2$ (ST+NP)             & 0.969          & \textbf{0.000} & \textbf{0.000} & 1.000          & \textbf{0.838} & 0.864          & 0.958          & 0.992          \\
%  $(SGD)^2$ (ST+CR)             & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & 0.940          & 0.885          & 0.889          & 0.955          & \textbf{0.984} \\
%  $(SGD)^2$ (ST+AR)             & 0.605          & \textbf{0.000} & 0.757          & 0.712          & 0.985          & 0.965          & 0.978          & 0.995          \\
%  $(SGD)^2$ (ST+IL+ANR)         & 0.603          & 0.725          & \textbf{0.000} & \textbf{0.421} & 0.935          & 0.961          & 0.973          & 0.997          \\
%  $(SGD)^2$ (IL+NP+VR)          & 0.323          & 0.143          & 0.954          & 0.963          & 0.913          & \textbf{0.631} & \textbf{0.926} & 0.991          \\
% \hline
% \end{tabular}
% \caption{\blue{Quality Measures of Crossing Angle Maximization}}
% \label{tab:quality-table-crossing_angle_maximization}
% \end{table*}



% %% ==== aspect_ratio ====
% \begin{table*}[thbp]
% \begin{tabular}{l|rrrrrrrr}
% \hline
%  methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
% \hline
%  neato                         & 0.062          & 0.145          & 0.483          & 0.010          & 0.143          & 0.314          & 0.065          & \textbf{0.012} \\
%  sfdp                          & 0.068          & 0.084          & 0.536          & 0.010          & 0.192          & 0.452          & 0.095          & 0.018          \\
%  $(SGD)^2$ (ST)                & 0.049          & 0.150          & 0.470          & \textbf{0.002} & 0.155          & 0.315          & 0.071          & 0.094          \\
%  $(SGD)^2$ (NP)                & \textbf{0.047} & 0.124          & 0.481          & 0.176          & 0.162          & \textbf{0.049} & 0.109          & 0.282          \\
%  $(SGD)^2$ (ST+NP)             & 0.049          & 0.126          & 0.479          & \textbf{0.002} & 0.192          & 0.209          & 0.077          & 0.101          \\
%  $(SGD)^2$ (ST+CR)             & 0.134          & 0.149          & 0.473          & 0.028          & 0.136          & 0.368          & \textbf{0.030} & 0.079          \\
%  $(SGD)^2$ (ST+AR)             & \textbf{0.047} & \textbf{0.017} & \textbf{0.048} & 0.008          & \textbf{0.118} & 0.154          & 0.043          & 0.057          \\
%  $(SGD)^2$ (ST+IL+ANR)         & \textbf{0.048} & 0.197          & 0.508          & 0.045          & 0.178          & 0.269          & 0.058          & 0.084          \\
%  $(SGD)^2$ (IL+NP+VR)          & 0.101          & 0.231          & 0.455          & 0.242          & 0.359          & 0.282          & 0.074          & 0.106          \\
% \hline
% \end{tabular}
% \caption{\blue{Quality Measures of Aspect Ratio}}
% \label{tab:quality-table-aspect_ratio}
% \end{table*}



% %% ==== angular_resolution ====
% \begin{table*}[thbp]
% \begin{tabular}{l|rrrrrrrr}
% \hline
%  methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
% \hline
%  neato                         & 0.753          & 0.749          & 0.525          & 0.999          & 0.998          & 1.000          & 1.000          & \textbf{1.000} \\
%  sfdp                          & 0.459          & 0.908          & 0.547          & 0.996          & 0.999          & 0.996          & 1.000          & \textbf{1.000} \\
%  $(SGD)^2$ (ST)                & \textbf{0.401} & 0.750          & 0.524          & 0.989          & \textbf{0.993} & 0.941          & 0.999          & \textbf{1.000} \\
%  $(SGD)^2$ (NP)                & 0.928          & 0.976          & 0.994          & 0.996          & 1.000          & 0.984          & 1.000          & \textbf{1.000} \\
%  $(SGD)^2$ (ST+NP)             & 0.952          & 0.466          & \textbf{0.487} & 1.000          & 0.999          & 0.998          & 0.999          & \textbf{1.000} \\
%  $(SGD)^2$ (ST+CR)             & 0.746          & 0.769          & 0.526          & 0.996          & 0.998          & 0.969          & \textbf{0.998} & \textbf{0.999} \\
%  $(SGD)^2$ (ST+AR)             & 0.403          & 0.779          & 0.991          & \textbf{0.963} & 0.998          & 0.994          & 0.999          & \textbf{1.000} \\
%  $(SGD)^2$ (ST+IL+ANR)         & \textbf{0.401} & \textbf{0.327} & 0.528          & 0.990          & 1.000          & \textbf{0.740} & \textbf{0.999} & \textbf{0.999} \\
%  $(SGD)^2$ (IL+NP+VR)          & 0.677          & 0.418          & 0.974          & 0.995          & 0.999          & 0.823          & \textbf{0.999} & \textbf{1.000} \\
% \hline
% \end{tabular}
% \caption{\blue{Quality Measures of Angular Resolution}}
% \label{tab:quality-table-angular_resolution}
% \end{table*}



% %% ==== vertex_resolution ====
% \begin{table*}[thbp]
% \begin{tabular}{l|rrrrrrrr}
% \hline
%  methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
% \hline
%  neato                         & 0.637          & 0.735          & \textbf{0.362} & 0.765          & 0.948          & 0.780          & 0.870          & \textbf{0.931} \\
%  sfdp                          & 0.391          & \textbf{0.594} & 0.807          & 0.825          & 0.951          & 0.877          & 0.859          & 0.967          \\
%  $(SGD)^2$ (ST)                & \textbf{0.269} & 0.727          & 0.368          & \textbf{0.663} & 0.991          & 0.798          & 0.869          & 0.976          \\
%  $(SGD)^2$ (NP)                & 1.000          & 0.875          & 0.902          & 0.992          & 0.986          & 0.814          & 0.827          & 0.987          \\
%  $(SGD)^2$ (ST+NP)             & 1.000          & 0.688          & 0.454          & 1.000          & 0.989          & 0.791          & 0.862          & 0.977          \\
%  $(SGD)^2$ (ST+CR)             & 0.570          & 0.762          & 0.379          & 0.789          & 0.954          & 0.908          & 0.785          & 0.950          \\
%  $(SGD)^2$ (ST+AR)             & 0.278          & 0.682          & 0.633          & 0.698          & 0.938          & 0.802          & 0.963          & 0.991          \\
%  $(SGD)^2$ (ST+IL+ANR)         & 0.332          & 0.959          & 0.392          & 0.873          & 0.961          & 0.959          & 0.931          & 0.984          \\
%  $(SGD)^2$ (IL+NP+VR)          & 0.355          & 0.615          & 0.795          & 0.744          & \textbf{0.831} & \textbf{0.590} & \textbf{0.751} & 0.993          \\
% \hline
% \end{tabular}
% \caption{\blue{Quality Measures of Vertex Resolution}}
% \label{tab:quality-table-vertex_resolution}
% \end{table*}



% %% ==== gabriel ====
% \begin{table*}[thbp]
% \begin{tabular}{l|rrrrrrrr}
% \hline
%  methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
% \hline
%  neato                         & 0.429          & 0.595          & \textbf{0.000} & 0.933          & \textbf{1.000} & 0.920          & \textbf{1.000} & \textbf{1.000} \\
%  sfdp                          & 0.860          & 0.806          & 0.148          & 0.758          & \textbf{1.000} & 0.967          & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (ST)                & 0.677          & \textbf{0.130} & \textbf{0.000} & 0.795          & \textbf{1.000} & 0.963          & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (NP)                & 0.951          & 0.954          & 0.973          & 0.920          & \textbf{1.000} & \textbf{0.903} & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (ST+NP)             & 0.951          & 0.658          & \textbf{0.000} & \textbf{0.039} & \textbf{1.000} & 0.916          & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (ST+CR)             & 0.704          & 0.205          & \textbf{0.000} & 0.967          & \textbf{1.000} & 0.988          & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (ST+AR)             & 0.678          & 0.396          & 0.887          & 0.903          & \textbf{1.000} & 0.958          & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (ST+IL+ANR)         & 0.681          & 0.745          & \textbf{0.000} & 0.630          & \textbf{1.000} & 0.967          & \textbf{1.000} & \textbf{1.000} \\
%  $(SGD)^2$ (IL+NP+VR)          & \textbf{0.421} & 0.800          & 0.982          & 0.926          & \textbf{1.000} & 0.972          & \textbf{1.000} & \textbf{1.000} \\
% \hline
% \end{tabular}
% \caption{\blue{Quality Measures of Gabriel}}
% \label{tab:quality-table-gabriel}
% \end{table*}

==> table-qualities.tex <==
%% ==== stress ====
\begin{table*}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.081          & \textbf{0.078} & \textbf{0.013} & \textbf{0.027} & 0.076          & \textbf{0.062} & 0.083          & \textbf{0.022} \\
 sfdp                          & 0.080 & 0.133          & 0.024          & 0.052          & 0.099          & 0.071          & \textbf{0.081} & 0.029          \\
 \GDGD (ST)                      & \textbf{0.079} & \textbf{0.078} & \textbf{0.013} & \textbf{0.027} & \textbf{0.071} & \textbf{0.062} & 0.082          & \textbf{0.022} \\
 \GDGD (NP)                      & 0.188          & 0.233          & 0.065          & 0.241          & 0.825          & 0.149          & 0.279          & 0.275          \\
 \GDGD (ST+IL)                   & 0.107          & 0.100          & 0.033          & 0.054          & 0.090          & 0.100          & 0.119          & 0.043          \\
 \GDGD (ST+NP)                   & 0.188          & 0.106          & \textbf{0.013} & 0.051          & 0.739          & 0.080          & 0.178          & 0.059          \\
 \GDGD (ST+CR)                   & 0.190          & \textbf{0.078} & \textbf{0.013} & 0.028          & 0.079          & 0.073          & 0.091          & 0.045          \\
 \GDGD (ST+CAM)                  & 0.099          & \textbf{0.078} & 0.015          & 0.029          & 0.075          & 0.063          & 0.094          & 0.029          \\
 \GDGD (ST+AR)                   & 0.080 & 0.081          & 0.055          & \textbf{0.027} & 0.075          & 0.067          & 0.084          & 0.023          \\
 \GDGD (ST+VR)                   & 0.083          & 0.080          & \textbf{0.013} & 0.032          & 0.073          & 0.063          & 0.088          & 0.023          \\
 \GDGD (ST+GB)                   & 0.080 & \textbf{0.078} & \textbf{0.013} & \textbf{0.027} & \textbf{0.071} & \textbf{0.062} & 0.083          & \textbf{0.022} \\
 \GDGD (ST+IL+ANR)               & 0.089          & 0.098          & 0.020          & 0.036          & 0.080          & 0.084          & 0.096          & 0.027          \\
 \GDGD (IL+NP+VR)                & 0.083          & 0.119          & 0.061          & 0.134          & 0.208          & 0.068          & 0.110          & 0.205          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Stress (ST)}}
\label{tab:quality-table-stress}
\end{table*}



%% ==== ideal_edge_length ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.028          & 0.005          & \textbf{0.002} & 0.099          & 0.484          & 0.026          & 0.299          & 0.280          \\
 sfdp                          & 0.018          & 0.143          & 0.051          & 0.271          & 0.585          & 0.052          & 0.279          & 0.346          \\
 \GDGD (ST)                      & 0.062          & 0.103          & 0.053          & 0.114          & 0.526          & 0.111          & 0.320          & 0.293          \\
 \GDGD (NP)                      & 0.679          & 0.867          & 0.351          & 0.884          & 3.348          & 0.649          & 1.083          & 1.312          \\
 \GDGD (ST+IL)                   & \textbf{0.004} & \textbf{0.003} & \textbf{0.002} & \textbf{0.009} & \textbf{0.462} & \textbf{0.002} & \textbf{0.249} & \textbf{0.245} \\
 \GDGD (ST+NP)                   & 0.679          & 0.227          & 0.056          & 0.434          & 1.608          & 0.418          & 0.749          & 0.519          \\
 \GDGD (ST+CR)                   & 0.517          & 0.103          & 0.053          & 0.139          & 0.593          & 0.205          & 0.394          & 0.482          \\
 \GDGD (ST+CAM)                  & 0.109          & 0.103          & 0.058          & 0.132          & 0.595          & 0.141          & 0.497          & 0.368          \\
 \GDGD (ST+AR)                   & 0.061          & 0.112          & 0.203          & 0.114          & 0.533          & 0.148          & 0.334          & 0.302          \\
 \GDGD (ST+VR)                   & 0.083          & 0.257          & 0.067          & 0.159          & 0.569          & 0.155          & 0.399          & 0.309          \\
 \GDGD (ST+GB)                   & 0.061          & 0.098          & 0.053          & 0.092          & 0.521          & 0.111          & 0.338          & 0.291          \\
 \GDGD (ST+IL+ANR)               & 0.016          & 0.027          & 0.012          & 0.029          & 0.486          & 0.027          & 0.277          & 0.268          \\
 \GDGD (IL+NP+VR)                & 0.082          & 0.178          & 0.116          & 0.242          & 0.702          & 0.147          & 0.388          & 0.549          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Ideal Edge Length (IL)}}
\label{tab:quality-table-ideal_edge_length}
\end{table}



%% ==== neighborhood_preservation ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.723          & 0.718          & \textbf{0.000} & 0.474          & 0.846          & 0.558          & 0.699          & 0.545          \\
 sfdp                          & 0.571          & 0.592          & 0.063          & 0.533          & 0.750          & 0.651          & 0.584          & 0.653          \\
 \GDGD (ST)                      & 0.500          & 0.721          & \textbf{0.000} & 0.503          & 0.832          & 0.553          & 0.657          & 0.548          \\
 \GDGD (NP)                      & \textbf{0.400} & 0.225          & 0.276          & 0.487          & \textbf{0.659} & 0.480          & \textbf{0.428} & 0.516          \\
 \GDGD (ST+IL)                   & 0.667          & 0.701          & \textbf{0.000} & 0.518          & 0.867          & 0.674          & 0.766          & 0.665          \\
 \GDGD (ST+NP)                   & \textbf{0.400} & \textbf{0.194} & \textbf{0.000} & 0.467          & 0.664          & \textbf{0.347} & 0.472          & \textbf{0.441} \\
 \GDGD (ST+CR)                   & 0.481          & 0.714          & \textbf{0.000} & \textbf{0.420} & 0.765          & 0.532          & 0.582          & 0.567          \\
 \GDGD (ST+CAM)                  & 0.681          & 0.721          & 0.042          & 0.531          & 0.851          & 0.552          & 0.763          & 0.631          \\
 \GDGD (ST+AR)                   & 0.500          & 0.727          & 0.418          & 0.492          & 0.842          & 0.560          & 0.757          & 0.584          \\
 \GDGD (ST+VR)                   & 0.750          & 0.708          & \textbf{0.000} & 0.609          & 0.834          & 0.527          & 0.709          & 0.570          \\
 \GDGD (ST+GB)                   & 0.696          & 0.727          & \textbf{0.000} & 0.566          & 0.831          & 0.555          & 0.702          & 0.547          \\
 \GDGD (ST+IL+ANR)               & 0.500          & 0.749          & \textbf{0.000} & 0.539          & 0.823          & 0.622          & 0.705          & 0.520          \\
 \GDGD (IL+NP+VR)                & 0.636          & \textbf{0.194} & 0.165          & 0.472          & 0.713          & 0.349          & 0.497          & 0.717          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Neighborhood Preservation (NP)}}
\label{tab:quality-table-neighborhood_preservation}
\end{table}



%% ==== crossings ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron & tree-2-6   & grid-12-24 & spx-teaser  & 494-bus      & grid1       & dwt-307      & dwt-1005      \\
\hline
 neato                         & 8            & 1          & \textbf{0} & 80          & 274          & 134         & 1896         & 8001          \\
 sfdp                          & 9            & 2          & \textbf{0} & \textbf{72} & 141          & 109         & 1651         & \textbf{5447} \\
 \GDGD (ST)                      & 10           & \textbf{0} & \textbf{0} & 73          & 283          & 133         & 1749         & 8367          \\
 \GDGD (NP)                      & 10           & 5          & 109        & 155         & 216          & \textbf{80} & 1251         & 10736         \\
 \GDGD (ST+IL)                   & 10           & \textbf{0} & \textbf{0} & 73          & 325          & 151         & 3924         & 13094         \\
 \GDGD (ST+NP)                   & 6            & \textbf{0} & \textbf{0} & 111         & \textbf{131} & 94          & \textbf{265} & 6932          \\
 \GDGD (ST+CR)                   & \textbf{0}   & \textbf{0} & \textbf{0} & 73          & 187          & 133         & 347          & 8827          \\
 \GDGD (ST+CAM)                  & 7            & \textbf{0} & 9          & 84          & 430          & 158         & 4673         & 12972         \\
 \GDGD (ST+AR)                   & 10           & \textbf{0} & 2          & \textbf{72} & 303          & 142         & 2836         & 8628          \\
 \GDGD (ST+VR)                   & 7            & \textbf{0} & \textbf{0} & 79          & 282          & 134         & 2983         & 8874          \\
 \GDGD (ST+GB)                   & 6            & \textbf{0} & \textbf{0} & 75          & 264          & 134         & 2034         & 8305          \\
 \GDGD (ST+IL+ANR)               & 10           & 24         & \textbf{0} & \textbf{72} & 302          & 171         & 2793         & 8241          \\
 \GDGD (IL+NP+VR)                & 6            & 2          & 96         & 105         & 173          & 103         & 1333         & 18276         \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Crossings (CR)}}
\label{tab:quality-table-crossings}
\end{table}



%% ==== crossing_angle_maximization ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.254          & 0.419          & \textbf{0.000} & 0.786          & 0.956          & 0.927          & 0.970          & 0.999          \\
 sfdp                          & 0.622          & 0.235          & \textbf{0.000} & 0.806          & 0.972          & 0.970          & 0.963          & 1.000          \\
 \GDGD (ST)                      & 0.601          & \textbf{0.000} & \textbf{0.000} & 0.975          & 0.923          & 0.946          & 0.983          & 0.990          \\
 \GDGD (NP)                      & 0.969          & 0.808          & 0.945          & 0.999          & 0.913          & 0.939          & 0.988          & 0.992          \\
 \GDGD (ST+IL)                   & 0.602          & \textbf{0.000} & \textbf{0.000} & 0.575          & 0.970          & 0.837          & 0.989          & 0.998          \\
 \GDGD (ST+NP)                   & 0.969          & \textbf{0.000} & \textbf{0.000} & 1.000          & \textbf{0.838} & 0.864          & 0.958          & 0.992          \\
 \GDGD (ST+CR)                   & \textbf{0.000} & \textbf{0.000} & \textbf{0.000} & 0.940          & 0.885          & 0.889          & 0.955          & \textbf{0.984} \\
 \GDGD (ST+CAM)                  & \textbf{0.000} & \textbf{0.000} & 0.810          & 0.646          & 0.937          & \textbf{0.622} & 0.973          & 0.993          \\
 \GDGD (ST+AR)                   & 0.605          & \textbf{0.000} & 0.757          & 0.712          & 0.985          & 0.965          & 0.978          & 0.995          \\
 \GDGD (ST+VR)                   & 0.164          & \textbf{0.000} & \textbf{0.000} & 0.550          & 0.943          & 0.883          & 0.975          & 0.995          \\
 \GDGD (ST+GB)                   & 0.524          & \textbf{0.000} & \textbf{0.000} & 0.834          & 0.945          & 0.937          & 0.992          & 0.991          \\
 \GDGD (ST+IL+ANR)               & 0.603          & 0.725          & \textbf{0.000} & \textbf{0.421} & 0.935          & 0.961          & 0.973          & 0.997          \\
 \GDGD (IL+NP+VR)                & 0.323          & 0.143          & 0.954          & 0.963          & 0.913          & 0.631          & \textbf{0.926} & 0.991          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Crossing Angle Maximization (CAM)}}
\label{tab:quality-table-crossing_angle_maximization}
\end{table}



%% ==== aspect_ratio ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.062          & 0.145          & 0.483          & 0.010          & 0.143          & 0.314          & 0.065          & \textbf{0.012} \\
 sfdp                          & 0.068          & 0.084          & 0.536          & 0.010          & 0.192          & 0.452          & 0.095          & 0.018          \\
 \GDGD (ST)                      & 0.049          & 0.150          & 0.470          & \textbf{0.002} & 0.155          & 0.315          & 0.071          & 0.094          \\
 \GDGD (NP)                      & \textbf{0.047} & 0.124          & 0.481          & 0.176          & 0.162          & \textbf{0.049} & 0.109          & 0.282          \\
 \GDGD (ST+IL)                   & \textbf{0.048} & 0.169          & 0.507          & 0.018          & 0.160          & 0.470          & 0.157          & 0.045          \\
 \GDGD (ST+NP)                   & 0.049          & 0.126          & 0.479          & \textbf{0.002} & 0.192          & 0.209          & 0.077          & 0.101          \\
 \GDGD (ST+CR)                   & 0.134          & 0.149          & 0.473          & 0.028          & 0.136          & 0.368          & 0.030          & 0.079          \\
 \GDGD (ST+CAM)                  & 0.068          & 0.149          & 0.449          & 0.009          & 0.188          & 0.288          & \textbf{0.028} & 0.141          \\
 \GDGD (ST+AR)                   & \textbf{0.047} & \textbf{0.017} & \textbf{0.048} & 0.008          & \textbf{0.118} & 0.154          & 0.043          & 0.057          \\
 \GDGD (ST+VR)                   & 0.068          & 0.135          & 0.466          & 0.009          & 0.152          & 0.300          & 0.044          & 0.091          \\
 \GDGD (ST+GB)                   & 0.069          & 0.154          & 0.470          & 0.013          & 0.155          & 0.318          & 0.037          & 0.093          \\
 \GDGD (ST+IL+ANR)               & \textbf{0.048} & 0.197          & 0.508          & 0.045          & 0.178          & 0.269          & 0.058          & 0.084          \\
 \GDGD (IL+NP+VR)                & 0.101          & 0.231          & 0.455          & 0.242          & 0.359          & 0.282          & 0.074          & 0.106          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Aspect Ratio (AR)}}
\label{tab:quality-table-aspect_ratio}
\end{table}



%% ==== angular_resolution ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.753          & 0.749          & 0.525          & 0.999          & 0.998          & 1.000          & 1.000          & \textbf{1.000} \\
 sfdp                          & 0.459          & 0.908          & 0.547          & 0.996          & 0.999          & 0.996          & 1.000          & \textbf{1.000} \\
 \GDGD (ST)                      & \textbf{0.401} & 0.750          & 0.524          & 0.989          & \textbf{0.993} & 0.941          & 0.999          & \textbf{1.000} \\
 \GDGD (NP)                      & 0.928          & 0.976          & 0.994          & 0.996          & 1.000          & 0.984          & 1.000          & \textbf{1.000} \\
 \GDGD (ST+IL)                   & 0.517          & 0.844          & 0.497          & 0.939          & 0.999          & 0.932          & 0.999          & \textbf{1.000} \\
 \GDGD (ST+NP)                   & 0.952          & 0.466          & \textbf{0.487} & 1.000          & 0.999          & 0.998          & 0.999          & \textbf{1.000} \\
 \GDGD (ST+CR)                   & 0.746          & 0.769          & 0.526          & 0.996          & 0.998          & 0.969          & \textbf{0.998} & \textbf{0.999} \\
 \GDGD (ST+CAM)                  & 1.000          & 0.745          & 0.871          & 0.913          & 1.000          & 0.999          & 1.000          & \textbf{0.999} \\
 \GDGD (ST+AR)                   & 0.403          & 0.779          & 0.991          & 0.963          & 0.998          & 0.994          & 0.999          & \textbf{1.000} \\
 \GDGD (ST+VR)                   & 0.760          & 0.979          & 0.540          & 0.936          & 1.000          & 0.914          & 1.000          & \textbf{1.000} \\
 \GDGD (ST+GB)                   & 0.573          & 0.750          & 0.528          & \textbf{0.868} & 1.000          & 0.903          & 1.000          & \textbf{1.000} \\
 \GDGD (ST+IL+ANR)               & \textbf{0.401} & \textbf{0.327} & 0.528          & 0.990          & 1.000          & \textbf{0.740} & \textbf{0.999} & \textbf{0.999} \\
 \GDGD (IL+NP+VR)                & 0.677          & 0.418          & 0.974          & 0.995          & 0.999          & 0.823          & \textbf{0.999} & \textbf{1.000} \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Angular Resolution (ANR)}}
\label{tab:quality-table-angular_resolution}
\end{table}



%% ==== vertex_resolution ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.637          & 0.735          & 0.362          & 0.765          & 0.948          & 0.780          & 0.870          & \textbf{0.931} \\
 sfdp                          & 0.391          & 0.594          & 0.807          & 0.825          & 0.951          & 0.877          & 0.859          & 0.967          \\
 \GDGD (ST)                      & 0.269          & 0.727          & 0.368          & 0.663          & 0.991          & 0.798          & 0.869          & 0.976          \\
 \GDGD (NP)                      & 1.000          & 0.875          & 0.902          & 0.992          & 0.986          & 0.814          & 0.827          & 0.987          \\
 \GDGD (ST+IL)                   & 0.334          & 0.705          & \textbf{0.354} & 0.788          & 0.993          & 0.973          & 0.994          & 0.993          \\
 \GDGD (ST+NP)                   & 1.000          & 0.688          & 0.454          & 1.000          & 0.989          & 0.791          & 0.862          & 0.977          \\
 \GDGD (ST+CR)                   & 0.570          & 0.762          & 0.379          & 0.789          & 0.954          & 0.908          & 0.785          & 0.950          \\
 \GDGD (ST+CAM)                  & 0.996          & 0.715          & 0.839          & 0.789          & 0.974          & 0.856          & 0.967          & 0.959          \\
 \GDGD (ST+AR)                   & 0.278          & 0.682          & 0.633          & 0.698          & 0.938          & 0.802          & 0.963          & 0.991          \\
 \GDGD (ST+VR)                   & \textbf{0.165} & \textbf{0.266} & 0.388          & \textbf{0.407} & \textbf{0.754} & \textbf{0.590} & \textbf{0.617} & 0.945          \\
 \GDGD (ST+GB)                   & 0.529          & 0.737          & 0.365          & 0.630          & 0.895          & 0.858          & 0.913          & 0.986          \\
 \GDGD (ST+IL+ANR)               & 0.332          & 0.959          & 0.392          & 0.873          & 0.961          & 0.959          & 0.931          & 0.984          \\
 \GDGD (IL+NP+VR)                & 0.355          & 0.615          & 0.795          & 0.744          & 0.831          & \textbf{0.590} & 0.751          & 0.993          \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Vertex Resolution (VR)}}
\label{tab:quality-table-vertex_resolution}
\end{table}



%% ==== gabriel ====
\begin{table}[h]
\color{blue}
\begin{tabular}{l|rrrrrrrr}
\hline
 methods \textbackslash~graphs & dodecahedron   & tree-2-6       & grid-12-24     & spx-teaser     & 494-bus        & grid1          & dwt-307        & dwt-1005       \\
\hline
 neato                         & 0.429          & 0.595          & \textbf{0.000} & 0.933          & \textbf{1.000} & 0.920          & \textbf{1.000} & \textbf{1.000} \\
 sfdp                          & 0.860          & 0.806          & 0.148          & 0.758          & \textbf{1.000} & 0.967          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST)                      & 0.677          & 0.130          & \textbf{0.000} & 0.795          & \textbf{1.000} & 0.963          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (NP)                      & 0.951          & 0.954          & 0.973          & 0.920          & \textbf{1.000} & 0.903          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+IL)                   & 0.679          & \textbf{0.000} & \textbf{0.000} & 0.834          & \textbf{1.000} & 0.860          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+NP)                   & 0.951          & 0.658          & \textbf{0.000} & \textbf{0.039} & \textbf{1.000} & 0.916          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+CR)                   & 0.704          & 0.205          & \textbf{0.000} & 0.967          & \textbf{1.000} & 0.988          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+CAM)                  & 0.695          & 0.199          & 0.799          & 0.836          & \textbf{1.000} & 0.905          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+AR)                   & 0.678          & 0.396          & 0.887          & 0.903          & \textbf{1.000} & 0.958          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+VR)                   & 0.437          & 0.957          & \textbf{0.000} & 0.862          & \textbf{1.000} & 0.987          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+GB)                   & \textbf{0.368} & 0.036          & \textbf{0.000} & 0.664          & \textbf{1.000} & \textbf{0.791} & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (ST+IL+ANR)               & 0.681          & 0.745          & \textbf{0.000} & 0.630          & \textbf{1.000} & 0.967          & \textbf{1.000} & \textbf{1.000} \\
 \GDGD (IL+NP+VR)                & 0.421          & 0.800          & 0.982          & 0.926          & \textbf{1.000} & 0.972          & \textbf{1.000} & \textbf{1.000} \\
\hline
\end{tabular}
\caption{\blue{Quality Measures of Gabriel Property (GB)}}
\label{tab:quality-table-gabriel}
\end{table}

